Efficient Deformable Tissue Reconstruction via Orthogonal Neural Plane

Intraoperative imaging techniques for reconstructing deformable tissues in vivo are pivotal for advanced surgical systems. Existing methods either compromise on rendering quality or are excessively computationally intensive, often demanding dozens of hours to perform, which significantly hinders their practical application. In this paper, we introduce Fast Orthogonal Plane (Forplane), a novel, efficient framework based on neural radiance fields (NeRF) for the reconstruction of deformable tissues. We conceptualize surgical procedures as 4D volumes, and break them down into static and dynamic fields comprised of orthogonal neural planes. This factorization iscretizes the four-dimensional space, leading to a decreased memory usage and faster optimization. A spatiotemporal importance sampling scheme is introduced to improve performance in regions with tool occlusion as well as large motions and accelerate training. An efficient ray marching method is applied to skip sampling among empty regions, significantly improving inference speed. Forplane accommodates both binocular and monocular endoscopy videos, demonstrating its extensive applicability and flexibility. Our experiments, carried out on two in vivo datasets, the EndoNeRF and Hamlyn datasets, demonstrate the effectiveness of our framework. In all cases, Forplane substantially accelerates both the optimization process (by over 100 times) and the inference process (by over 15 times) while maintaining or even improving the quality across a variety of non-rigid deformations. This significant performance improvement promises to be a valuable asset for future intraoperative surgical applications. The code of our project is now available at https://github.com/Loping151/ForPlane.

==> 4_results.tex <==
\section{Guidelines for Graphics Preparation and Submission}
\label{sec:guidelines}

\subsection{Types of Graphics}
The following list outlines the different types of graphics published in 
IEEE journals. They are categorized based on their construction, and use of 
color~/~shades of gray:

\subsubsection{Color/Grayscale figures}
{Figures meant to appear in color, or shades of black/gray. Such 
figures may include photographs, illustrations, multicolor graphs, and 
flowcharts.}

\subsubsection{Line Art figures}
{Figures that are composed of only black lines and shapes. These figures 
should have no shades or half-tones of gray, only black and white.}

\subsubsection{Author photos}
{Not allowed for papers in TMI.}

\subsubsection{Tables}
{Data charts which are typically black and white, but sometimes include 
color.}

\begin{table}
\caption{Units for Magnetic Properties}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
\hline
Symbol& 
Quantity& 
Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
\hline
$\Phi $& 
magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
$B$& 
magnetic flux density, \par magnetic induction& 
1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
$H$& 
magnetic field strength& 
1 Oe $\to  10^{3}/(4\pi )$ A/m \\
$m$& 
magnetic moment& 
1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
$M$& 
magnetization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
4$\pi M$& 
magnetization& 
1 G $\to  10^{3}/(4\pi )$ A/m \\
$\sigma $& 
specific magnetization& 
1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
$j$& 
magnetic dipole \par moment& 
1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
$J$& 
magnetic polarization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
$\chi , \kappa $& 
susceptibility& 
1 $\to  4\pi $ \\
$\chi_{\rho }$& 
mass susceptibility& 
1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
$\mu $& 
permeability& 
1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
$\mu_{r}$& 
relative permeability& 
$\mu \to \mu_{r}$ \\
$w, W$& 
energy density& 
1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
$N, D$& 
demagnetizing factor& 
1 $\to  1/(4\pi )$ \\
\hline
\multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
the entire table do not need footnote letters. }\\
\multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
$=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
kilogram, H $=$ henry.}
\end{tabular}
\label{tab1}
\end{table}

\subsection{Multipart figures}
Multipart figures are comprised of more than one sub-figure presented together.
If a multipart figure is made up of multiple figure types (one part is lineart,
and another is grayscale or color) the figure should meet the strictest applicable guidelines.

\subsection{File Formats For Graphics}
\label{formats}
Format and save your graphics as one of the following approved file types:
PostScript (.PS), Encapsulated PostScript (.EPS), Tagged Image File Format (.TIFF),
Portable Document Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS).
After the paper is accepted, any included graphics must be submitted alongside the final manuscript files.

\subsection{Sizing of Graphics}
Most charts, graphs, and tables are one column wide (3.5 inches~/~88 
millimeters) or page wide (7.16 inches~/~181 millimeters). The maximum
depth of a graphic is 8.5 inches (216 millimeters). When choosing the depth of a graphic,
please allow space for a caption. Authors are allowed to size figures between column and
page widths, but it is recommended not to size figures less than column width unless necessary. 

\subsection{Resolution}
The proper resolution of your figures will depend on the type of figure it 
is as defined in the ``Types of Figures'' section. Author photographs, 
color, and grayscale figures should be at least 300dpi. Lineart, including 
tables should be a minimum of 600dpi.

\subsection{Vector Art}
While IEEE does accept and even recommends that authors submit artwork
in vector format, it is our policy is to rasterize all figures for publication. This is done
in order to preserve figures' integrity across multiple computer platforms.

\subsection{Colorspace}
The term colorspace refers to the entire sum of colors that can be 
represented within a given medium. For our purposes, the three main colorspaces
are grayscale, RGB (red/green/blue) and CMYK (cyan/magenta/yellow/black).
RGB is generally used with on-screen graphics, whereas CMYK is used for printing purposes.

All color figures should be generated in RGB or CMYK colorspace. Grayscale 
images should be submitted in grayscale colorspace. Line art may be 
provided in grayscale OR bitmap colorspace. Note that ``bitmap colorspace'' 
and ``bitmap file format'' are not the same thing. When bitmap colorspace 
is selected, .TIF/.TIFF are the recommended file formats.

\subsection{Accepted Fonts Within Figures}
When preparing your graphics IEEE suggests that you use of one of the 
following Open Type fonts: Times New Roman, Helvetica, Arial, Cambria, and 
Symbol. If you are supplying EPS, PS, or PDF files all fonts must be 
embedded. Some fonts may only be native to your operating system; without 
the fonts embedded, parts of the graphic may be distorted or missing.

A safe option when finalizing your figures is to strip out the fonts before 
you save the files, creating ``outline'' type. This converts fonts to 
artwork that will appear uniformly on any screen.

\subsection{Using Labels Within Figures}

\subsubsection{Figure Axis labels}
Figure axis labels are often a source of confusion. Use words rather than 
symbols. As an example, write the quantity ``Magnetization,'' or 
``Magnetization M,'' not just ``M.'' Put units in parentheses. Do not label 
axes only with units. As in Fig. 1, for example, write ``Magnetization 
(A/m)'' or ``Magnetization (A$\cdot$m$^{-1}$),'' not just ``A/m.''
Do not label axes with a ratio of quantities and units.
For example, write ``Temperature (K),'' not ``Temperature/K.'' 

Multipliers can be especially confusing. Write ``Magnetization (kA/m)'' or 
``Magnetization (10$^{3}$ A/m).'' Do not write ``Magnetization 
(A/m)$\,\times\,$1000'' because the reader would not know whether the top 
axis label in Fig. 1 meant 16000 A/m or 0.016 A/m. Figure labels should be 
legible, approximately 8 to 10 point type.

\subsubsection{Subfigure Labels in Multipart Figures and Tables}
Multipart figures should be combined and labeled before final submission. 
Labels should appear centered below each subfigure in 8 point Times New 
Roman font in the format of (a) (b) (c).

\subsection{Referencing a Figure or Table Within Your Paper}
When referencing your figures and tables within your paper, use the 
abbreviation ``Fig.'' even at the beginning of a sentence. Do not abbreviate 
``Table.'' Tables should be numbered with Roman numerals.

\subsection{Submitting Your Graphics}
Format your paper with the graphics included within the body of the text
as you would expect to see the paper in print. Please do this at each stage of the review,
from first submission to final files. For final files only, after the paper has been accepted
for publication, figures should also be submitted individually in addition to the manuscript
file using one of the approved file formats. Place a figure caption below each figure;
place table titles above the tables. Do not include captions or borders in the uploaded figure files.

\subsection{File Naming}
Figures (line artwork or images) should be named starting with the 
first 5 letters of the corresponding author's last name. The next characters in the 
filename should be the number that represents the figure's sequential 
location in the article. For example, in author ``Anderson's'' paper,
the first three figures might be named ander1.tif, ander2.tif, and ander3.ps.

Tables should contain only the body of the table (not the caption) and 
should be named similarly to figures, except that `.t' is inserted 
in-between the author's name and the table number. For example, author 
Anderson's first three tables would be named ander.t1.tif, ander.t2.ps, ander.t3.eps.

Author photographs or biographies are not permitted in IEEE TMI papers.

\subsection{Checking Your Figures: The IEEE Graphics Analyzer}
The IEEE Graphics Analyzer enables authors to pre-screen their graphics for 
compliance with IEEE Transactions and Journals standards before submission. 
The online tool, located at \underline{http://graphicsqc.ieee.org/},
allows authors to upload their graphics in order to check that each file is the correct file format,
resolution, size and colorspace; that no fonts are missing or corrupt;
that figures are not compiled in layers or have transparency,
and that they are named according to the IEEE Transactions and Journals naming convention.
At the end of this automated process, authors are provided with 
a detailed report on each graphic within the web applet, as well as by email.

For more information on using the Graphics Analyzer or any other graphics 
related topic, contact the IEEE Graphics Help Desk by e-mail at 
graphics@ieee.org.

\subsection{Color Processing/Printing in IEEE Journals}
All IEEE Transactions, Journals, and Letters allow an author to publish 
color figures on IEEE Xplore\textregistered\ at no charge, and automatically 
convert them to grayscale for print versions. In most journals, figures and 
tables may alternatively be printed in color if an author chooses to do so. 
Please note that this service comes at an extra expense to the author. If 
you intend to have print color graphics, include a note with your final 
paper indicating which figures or tables you would like to be handled that way,
and stating that you are willing to pay the additional fee.

\section{Some Common Mistakes}
The word ``data'' is plural, not singular. The subscript for the 
permeability of vacuum $\mu _{0}$ is zero, not a lowercase letter 
``o.'' Use the word ``micrometer'' instead of ``micron.'' A graph within a graph is an 
``inset,'' not an ``insert.'' The word ``alternatively'' is preferred to the 
word ``alternately'' (unless you really mean something that alternates). Use 
the word ``whereas'' instead of ``while'' (unless you are referring to 
simultaneous events). Do not use the word ``essentially'' to mean 
``approximately'' or ``effectively.'' Do not use the word ``issue'' as a 
euphemism for ``problem.'' When compositions are not specified, separate 
chemical symbols by en-dashes; for example, ``NiMn'' indicates the 
intermetallic compound Ni$_{0.5}$Mn$_{0.5}$ whereas 
``Ni--Mn'' indicates an alloy of some composition 
Ni$_{x}$Mn$_{1-x}$.

Be aware of the different meanings of the homophones ``affect'' (usually a 
verb) and ``effect'' (usually a noun), ``complement'' and ``compliment,'' 
``discreet'' and ``discrete,'' ``principal'' (e.g., ``principal 
investigator'') and ``principle'' (e.g., ``principle of measurement''). Do 
not confuse ``imply'' and ``infer.'' 

Prefixes such as ``non,'' ``sub,'' ``micro,'' ``multi,'' and ``ultra'' are 
not independent words; they should be joined to the words they modify, 
usually without a hyphen. There is no period after the ``et'' in the Latin 
abbreviation ``\emph{et al.}'' (it is also italicized). The abbreviation ``i.e.,'' means 
``that is,'' and the abbreviation ``e.g.,'' means ``for example'' (these 
abbreviations are not italicized).

A general IEEE styleguide is available at \underline{http://www.ieee.org/web/publications/authors/transjnl/index.ht}
\discretionary{}{}{}\underline{ml}.

==> LaTeX/0_abstract.tex <==
\begin{abstract}
% Developing high-fidelity and fast algorithms for reconstructing deformable tissues among surgical procedures is one of the main research fields in computer-assisted surgery and endoscopy. 
% Existing methods either compromise on rendering quality or are excessively computationally intensive, often demanding dozens of hours to perform, which significantly hinders their practical application.
% In this paper, we propose an novel efficient framework named Fast Orthogonal Plane (Forplane) for the reconstruction of deformable tissues.
% Forplane leverages the implicit representation together with the volume rendering technology to represent the complex surgical procedures, which have been proved its effectiveness.
% We treats surgical procedures as 4D volumes and factorizes them into a combination of static and dynamic fields, which consists of orthogonal neural planes. This factorization discretization the four-dimensional space, leading to a compact memory footprint and reduce the number of parameters that need to be optimized. Besides, the time-invariant static field enables sharing information across frames, simplifying the difficulty of optimization.
% A novel sample scheme to boost optimization and improve performance in regions with tool occlusion and large motions.
% In this extended journal paper, we design an efficient ray marching algorithm to boost the rendering speed, and introduce a monocular version named MForplane to support various endoscopic videos. 
% Sufficient experiments are performed on two in vivo datasets, EndoNeRF dataset and Hamlyn dataset. 
% In all these cases, our framework significantly accelerates optimization by over 100$\times$ and inference by over 
% 12$\times$ while maintaining or even superior quality across various non-rigid deformations, showing significant promise for future intraoperative surgery applications. 

% Intraoperative imaging techniques for obtaining the shape and morphology of soft-tissue surfaces in vivo are a key enabling technology for advanced surgical systems. 

% The development of fast, high-fidelity algorithms for the reconstruction of deformable tissues in surgical procedures is a primary area of study in computer-assisted surgery and endoscopy. 

Intraoperative imaging techniques for reconstructing deformable tissues in vivo are pivotal for advanced surgical systems. 
Existing methods either compromise on rendering quality or are excessively computationally intensive, often demanding dozens of hours to perform, which significantly hinders their practical application.
In this paper, we introduce Fast Orthogonal Plane (Forplane), a novel, efficient framework based on neural radiance fields (NeRF) for the reconstruction of deformable tissues. 
% In this paper, we introduce Fast Orthogonal Plane (Forplane), a novel, efficient framework for the reconstruction of deformable tissues. Forplane combines implicit representation and volume rendering to accurately represent complex surgical procedures. 
We conceptualize surgical procedures as 4D volumes, and break them down into static and dynamic fields comprised of orthogonal neural planes. This factorization discretizes the four-dimensional space, leading to a decreased memory usage and faster optimization. 
A spatiotemporal importance sampling scheme is introduced to improve performance in regions with tool occlusion as well as large motions and accelerate training.
An efficient ray marching method is applied to skip sampling among empty regions, significantly improving inference speed.
% Considerable efforts have been dedicated to enhancing the rendering quality, optimization, and inference speed, which involve the implementation of new sampling scheme, efficient ray marching technique, and spatiotemporal information enhancement.
% A novel sampling scheme is used to boost optimization and improve performance in regions with tool occlusion and large motions.
% The time-invariant static field facilitates information sharing across frames, simplifying optimization.
% Besides, we propose a novel sample scheme to boost optimization and improve performance in regions with tool occlusion and large motions.
% One efficient ray marching algorithm is applied to accelerate the inference.
% We also introduce a monocular version, MForplane, to accommodate various endoscopic videos without sacrificing reconstruction quality.
Forplane accommodates both binocular and monocular endoscopy videos, demonstrating its extensive applicability and flexibility.
Our experiments, carried out on two in vivo datasets, the EndoNeRF and Hamlyn datasets, demonstrate the effectiveness of our framework. In all cases, Forplane substantially accelerates both the optimization process (by over 100 times) and the inference process (by over 15 times) while maintaining or even improving the quality across a variety of non-rigid deformations. This significant performance improvement promises to be a valuable asset for future intraoperative surgical applications. The code of our project is now available at \href{https://github.com/Loping151/ForPlane}{https://github.com/Loping151/ForPlane}.

% Our TiNeuVox completes training with only 8 minutes and 8-MB storage cost while showing similar or even better rendering performance than previous dynamic NeRF methods.
% the RSTN outperforms the baseline (a stagewise coarse-to-ﬁne approach) signiﬁcantly.
% several CT datasets including a public pancreas segmentation dataset, our own multi-organ dataset, and a cystic pancreas dataset. In all these cases, the RSTN outperforms the baseline (a stagewise coarse-to-ﬁne approach) signiﬁcantly.
% Our framework significantly accelerates the optimization of dynamic radiance fields while maintaining high rendering quality. Empirical evaluation is performed on both synthetic and real scenes. Our TiNeuVox completes training with only 8 minutes and 8-MB storage cost while showing similar or even better rendering performance than previous dynamic NeRF methods.
% Forplane treats surgical procedures as 4D volumes and factorizes them into explicit 2D planes of static and dynamic fields, leading to a compact memory footprint and significantly accelerated optimization. 
% The efficient factorization is accomplished by fusing features obtained through linear interpolation of each plane and enables using lightweight neural networks to model surgical scenes. Besides, Forplane shares static fields, significantly reducing the workload of dynamic tissue modeling.
% We also propose a novel sample scheme to boost optimization and improve performance in regions with tool occlusion and large motions. Experiments on DaVinci robotic surgery videos demonstrate that Forplane accelerates optimization by over 100$\times$ while maintaining high quality across various non-rigid deformations, showing significant promise for future intraoperative surgery applications. 
% Forplane factorizes 4D volumes into static and dynamic fields comprising explicit 2D planes, resulting in a compact memory footprint and significantly accelerated optimization. 
% This factorization is achieved by fusing the features obtained from the linear interpolation of each plane, which is highly efficient. This efficient spatial representation also enables us to use the tiny neural network to model the surgical process.
% With static fields, Forplane significantly reduces the workload of modeling dynamic tissues.
% By fusing vectors from spatiotemporal planes using linear interpolation, Forplane efficiently computes features for spatiotemporal points.
% By sharing static fields, lerp-lane significantly reduces the workload of modeling dynamic organizations.
% Thanks to the efficient feature representation, Forplane can use Tiny MLP to model the space, effectively accelerating the calculation.
% Code will be available 
% Forplane fuses vectors from spatiotemporal planes using linear interpolation to compute features for spatiotemporal points and uses volume rendering to render color and depth. 
%%%%%%%%%%%%%
% We propose a new approach, Forplane, for rapidly reconstructing deformable tissues during surgical procedures. Forplane leverages orthogonal planes to represent dynamic 4D space, achieving performance comparable to the current SOTA with just 3 minutes of optimization. This is over 100x faster than existing methods for a single procedure. Importantly, Forplane achieves faster optimization without sacrificing reconstruction quality, which suggests its potential for future clinical applications.
% In this extended journal paper, we allow a gradual optimization to improve the stability of the RSTN, and introduce a hierarchical version named H-RSTN to segment tiny and variable neoplasms such as pancreatic cysts. Experiments are performed on several CT datasets including a public pancreas segmentation dataset, our own multi-organ dataset, and a cystic pancreas dataset. In all these cases, the RSTN outperforms the baseline (a stagewise coarse-to-ﬁne approach) signiﬁcantly.
%%%%%%%%%%%%%%
% \keywords{Fast 3D Reconstruction \and Neural Rendering \and Robotic Surgery.}
\end{abstract}
\begin{IEEEkeywords}
Endoscopy, tissues reconstruction, optical imaging.
\end{IEEEkeywords}

==> LaTeX/1_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% \subsection{Motivation}
% \IEEEPARstart{R}{econstructing} deformable tissues from monocular endoscopic videos in surgery is an important and promising area in medical image computing. This particular field holds significant promise for facilitating a wide range of applications, encompassing enhanced surgical visual cognition, educational advancements in robotic surgery, and augmented situational awareness during intraoperative interventions.
% Real-time reconstruction is a fundamental component in these applications, providing a panoramic view of the surgical environment. This comprehensive visualization is pivotal in enabling precise manipulation of surgical instruments and minimizing errors in intricate surgical procedures. 
% However, the complex nature of surgical environments poses challenges, characterized by areas of restricted visibility and intricate structures, such as blood vessels and nerves. Successful surgical procedures necessitate clear identification and visualization of pathologies, such as tumors or enlarged lymph nodes. The fast and effective reconstruction of deformable tissues offers a viable solution for these challenges. By capturing intricate tissue details during surgery, this approach minimizes the need for invasive post-operative interventions while overcoming visual constraints within restricted surgical domains. Consequently, it enhances surgical planning and execution, leading to improved patient outcomes. This research paper specifically focuses on the fast reconstruction of deformable tissues within the context of endoscopy videos, encompassing all the aforementioned challenges and opportunities.
% \IEEEPARstart{R}{econstructing} deformable tissues from monocular endoscopy videos in surgery is an important and promising area in medical image computing that enables a wide range of applications. Effective surgery requires precise identification and visualization of pathologies, including tumors and enlarged lymph nodes. 
% However, limited visibility and complex structures, such as blood vessels and nerves, pose significant challenges on the high-quality visualization. Rapid and accurate reconstruction of deformable tissues during surgery addresses these constraints and minimizes invasiveness within restricted surgical domains. 
% It captures intricate tissue details, enhancing surgical planning, execution, and ultimately improving patient outcomes. This paper specifically targets fast reconstruction of deformable tissues in monocular endoscopy videos, encompassing the aforementioned challenges and opportunities.
\IEEEPARstart{R}{econstructing} deformable tissues from endoscopy videos in surgery is a crucial and promising field in medical image computing. High-quality tissue reconstruction can assist surgeons in avoiding critical structures, \textit{e.g.}, blood vessels and nerves, as well as improve the observation of lesions such as tumors and enlarged lymph nodes~\cite{https://doi.org/10.1111/iju.14038, BIANCHI2020e669}. Moreover, tissue reconstruction significantly contributes to creating a virtual surgical training environment~\cite{LANGE200061}. Such detailed reconstructions not only facilitate skill acquisition and expedite the learning curve for endoscopists but also generate substantial training data. This data is crucial for developing virtual reality (VR) and augmented reality (AR) training modules in surgical education, as well as for enhancing the learning algorithms of surgical robots~\cite{9807505, long2022robotic}.
However, achieving precise identification and visualization of these structures and lesions remains a challenge for existing methods. Moreover, the extensive training and inference time required by these methods hinders their practical application during surgery.
This paper aims to address these challenges and seize the opportunities by focusing on high-quality real-time reconstruction of deformable tissues in both monocular and binocular endoscopy videos, providing valuable insights for future intraoperative applications.

% deformable tissues from monocular endoscopy videos in surgery is an important and promising area in medical image computing. High quality tissue reconstruction can help surgeons avoid blood vessels, nerves, and important structures, while also better observing lesions including tumors and enlarged lymph nodes. To achieve this, precise identification and visualization of the structures and lesions are required, which existing methods can reach. Besides, hours of training time these methods consume make it difficult for intraoperative use. This paper specifically targets high-quality real-time reconstruction of deformable tissues in monocular endoscopy videos, encompassing the aforementioned challenges and opportunities.
% 介绍general task的application
%% High quality tissue reconstruction can help surgeons avoid blood vessels, nerves, and important structures, while also better observing lesions such as tumors, ischemic necrotic lesions, and enlarged lymph nodes.

% 介绍具体的task setting
%% 例子：This paper focuses on the specific setting of recovering the 6DoF pose of an object, i.e., rotation and translation in 3D, from a single RGB image of that object.
% This paper focuses on the specific setting of recovering/reconstructing/estimating [xxx 输出] from [xxx 输入].

Previous methods~\cite{maier2014comparative, mahmoud2018live, semmler20163d, luegmair2015three} primarily focus on static surgical scenes and disregard the presence of diverse surgical instruments in endoscopy videos. These methods rely on simultaneous localization and mapping (SLAM) techniques, generating individual meshes for each frame to reconstruct surgical procedures. However, they fail to account for non-rigid transformations in deformable tissues and potential occlusions caused by surgical instruments. As a result, their reconstruction performance lacks fidelity, contains gaps, and does not realistically represent the surgical environment. These limitations significantly hinder their applicability in data simulation and intraoperative assistance.

\begin{figure*}[ht]
\centerline{\includegraphics[width=0.95\textwidth]{figures/curve.png}}
% \vspace{-0.5em}
\caption{A) The speed-quality comparison between our Forplane and EndoNeRF~\cite{endonerf}. 
We present the performance of the two methods in terms of PSNR and provide insights into their training times. Furthermore, we showcase the reconstruction results obtained from both methods at various training time intervals, specifically at 3, 6, 9, and 12 minutes. These results clearly demonstrate the significant convergence speed exhibited by Forplane.
B) The metrics (PSNR, SSIM) of 7 different methods on the $\textit{pushing tissues}$ scene from EndoNeRF dataset~\cite{endonerf}. 
Both metrics exhibit a positive correlation, indicating that higher values shows better performance.
% A) Comparative optimization performance (time-PSNR) of Forplane and EndoNeRF. We compare the optimization efficiency of the two methods by comparing the time-PSNR curves and provide images obtained using different methods with the same optimization time. B) We conduct a performance analysis (PSNR) of various methods on the EndoNeRF dataset, which is represented as a box plot. Among them, our method exhibit a higher mean performance.
}
% \vspace{2em}
\label{fig: figcurve}
\end{figure*}

% We introduce the NeRF-based methods.
Recently, the integration of implicit scene representations and differentiable volume rendering has exhibited remarkable efficacy in capturing complex scenarios.
A notable example is neural radiance fields (NeRF)~\cite{nerf}, a seminal work in neural rendering that introduced neural implicit fields for continuous scene representations. NeRF has demonstrated exceptional performance in tasks such as high-quality view synthesis and 3D reconstruction across diverse contexts~\cite{xie2022neural}. Furthermore, NeRF and its variants have showcased diverse applications in medical imaging, encompassing but not restricted to medical imaging segmentation~\cite{khan2022implicit}, deformable tissue reconstruction~\cite{endonerf, lerplane}, radiograph measurement reconstruction~\cite{li20213d, corona2022mednerf}, and organ shape completion~\cite{yang2022implicitatlas, ruckert2022neat}.

% introduce endonerf
A notable advancement in reconstructing deformable tissue is EndoNeRF~\cite{endonerf}, a recent approach that has demonstrated exceptional capabilities in 3D reconstruction and deformation tracking of surgical scenes within the context of robotic surgery. EndoNeRF~\cite{endonerf} employs a canonical neural radiance field in conjunction with a time-dependent neural displacement field to effectively model deformable tissues using binocular captures within a single viewpoint configuration. However, despite its impressive achievements in reconstructing deformable tissues, EndoNeRF~\cite{endonerf} faces computational challenges due to intensive optimization processes. The optimization process for EndoNeRF~\cite{endonerf} typically requires tens of hours to complete, as each pixel generated necessitates a substantial number of neural network calls. This computational bottleneck significantly restricts the widespread adoption of such methods in surgical procedures.
Additionally, its performance heavily relies on precise binocular depth estimation, further impeding its broader applications.
% claim the improvements
% Several explicit and hybrid methods have been developed to model static scenes, achieving notable speed improvements over NeRF by utilizing explicit spatial data structures or features decoded by small MLPs. However, these methods have thus far been exclusively applied to static scenes. Applying these methods to surgical scenes presents significant challenges for two primary reasons. Firstly, encoding temporal information is crucial for modeling surgical scenes. Nevertheless, naively adding a temporal dimension to the explicit data structure can substantially escalate memory and computational requirements. Secondly, dynamic surgical scene reconstruction encounters limitations in viewpoints, often providing only one view per timestep, unlike static scenes that can leverage multi-view consistency for enhanced regularization. Consequently, this condition necessitates the sharing of information across disjoint timesteps to improve reconstruction quality.


% claim our method
To overcome the challenges mentioned above, we propose a novel approach called Forplane (Fast Orthogonal Plane), which delivers efficient and high-quality deformable tissue reconstruction and offers rapid training and inference with endoscopy videos. Forplane integrates space-time decomposition with neural radiance fields to achieve rapid and accurate reconstruction of deformable tissues during surgical procedures. By treating surgical procedures as 4D volumes, with time as an orthogonal axis to spatial coordinates, Forplane discretizes the continuous space into static and dynamic fields. Static fields are represented by spatial planes, while dynamic fields are represented by space-time planes.
We utilize limited resolution features to represent these planes, allowing for bilinear interpolation when querying features at any spatio-temporal point. This design markedly reduces computational costs compared to MLP-reliant methods~\cite{park2021nerfies, pumarola2021d, endonerf}, cutting down complexity from O$(N^4)$ to O$(N^2)$.
Additionally, the static field facilitates information sharing across neighboring timesteps, addressing the limitations imposed by restricted viewpoints. 
Furthermore, drawing inspiration from the observation that certain tissues exhibit more frequent deformations, we develope an importance sampling method, which strategically higher sampling probability towards tissues that are either occluded by surgical tools or exhibit more extensive motion range.
% \rep{Recognizing that certain tissues undergo more frequent deformation, our approach analyzes the temporal dynamics of the training data to identify these high-motion regions. We then allocate increased sampling probability to these ``challenging'' tissues. This targeted strategy not only enhances Forplane's focus on complex deformations but also facilitates faster convergence and improved overall reconstruction efficiency.}


A preliminary version of Forplane was introduced in Lerplane~\cite{lerplane}, where its ability to achieve rapid reconstruction of deformable tissues on binocular endoscopy videos was demonstrated. 
\textbf{1) Advancements in Rendering and Speed}: In this extended version, we have made notable advancements on rendering quality, inference speed and adaptability.
Specifically, we develop an efficient ray marching algorithm to guide the rendering procedure, significantly improving inference speed and rendering quality.
% Due to size constraints, current minimally invasive surgeries predominantly utilize monocular devices.
\textbf{2) MForplane for Monocular Videos}: Considering that many surgical procedures employ monocular devices, we present MForplane, a version of Forplane adapted for monocular videos.
MForplane performs effectively on monocular sequences alone with minimal performance drop, though this is a more challenging task.
% To enhance the adaptability of our method, we have developed an advanced optimization algorithm based on monocular depth estimation. This enhancement enables Forplane to generate high-quality dynamic tissue reconstructions, even when working with monocular sequences alone. We specifically refer to the variant of Forplane optimized for monocular sequences as MForplane.
\textbf{3) Comprehensive Evaluation with Hamlyn Datasets}: In addition to validating our results with the EndoNeRF dataset~\cite{endonerf}, we have expanded our evaluation to include the public Hamlyn dataset~\cite{hamlyn1,hamlyn2}. This dataset offers more complex sequences that encompass various challenging factors such as intracorporeal scenes with weak textures, deformations, motion blur, reflections, surgical tools, and occlusions. The inclusion of this dataset allows us to assess the performance of Forplane in more diverse and realistic surgical scenarios.
Fig.~\ref{fig: figcurve} shows that Forplane excels in its significantly faster optimization, demonstrating superior quantitative and qualitative performance in 3D reconstruction and deformation tracking within surgical scenes in comparison to preceding methods. 
Fig~\ref{fig: our performance a} demonstrates the superior reconstruction quality of Forplane.
These results herald significant potential for future intraoperative applications.

The remainder of this paper is organized as follows. Section II provides a concise review of the literature pertinent to our domain. Section III delineates the principal components of our Forplane framework. Section IV details the experimental results, validating the efficacy of our approach. In Section V, we elucidate the mechanisms underlying Forplane's capacity for efficient reconstruction of deformable tissues and outlines future research directions. Finally, Section VI synthesizes our findings and contributions into a conclusion.


% we draw inspiration from explicit data structure and propose a novel approach termed Forplane (Fast Orthogonal Plane) to achieve fast and accurate reconstruction of deformable tissues in surgical procedures.
% Specifically, we consider surgical procedures as 4D volumes, where the time axis is orthogonal to the 3D spatial coordinates.
% To Discretization continuous space to reduce computation, we decompose these 4D volumes into 2D planes. Forplane employs spatial planes to represent static fields and space-time planes to represent dynamic fields. This factorization strategy not only results in a compact memory footprint but also significantly accelerates the optimization process when compared to previous methods that solely relied on multilayer perceptrons (MLPs). Additionally, Forplane facilitates information sharing across different timesteps within the static field, thereby alleviating the limitations imposed by restricted viewpoints.
% By factorizing 4D volumes into 2D planes, Forplane utilizes space planes to represent static fields and space-time planes to represent dynamic fields. This factorization yields a compact memory footprint and significantly speeds up the optimization process compared to previous methods solely relying on MLPs. Additionally, Forplane facilitates information sharing across timesteps within the static field, thereby mitigating the negative impact of limited viewpoints.
% To optimize the neural linear planes efficiently and mitigate the influence of surgical instrument occlusion, Forplane introduces a novel sampling approach based on tool masks and contents. This approach assigns higher sampling probability to tissue pixels occluded by instruments or exhibiting a wider range of motion. 


% A previous iteration of Forplane was introduced in a conference paper~\cite{lerplane}, wherein its capability for swift deformable tissue reconstruction was ascertained. In this extended version of the study, we have made strides towards enhancing optimization and inference speeds, as well as rendering quality, facilitated by an auxiliary sampling network. To improve the adaptability of our method, we have devised an advanced optimization algorithm grounded in monocular depth estimation techniques. This allows Forplane to generate high-quality dynamic tissue reconstructions, even in scenarios limited to monocular sequences. We designate the Forplane variant optimized with monocular sequences as Forplane$\_$mono. Besides corroborating our results with the original EndoNeRF dataset, we expanded our evaluation to encompass the public Hamlyn dataset, which provides more complex sequences featuring intracorporeal scenes with weak textures, deformations, motion blur, reflections, surgical tools, and occlusions.

% Our contributions can be summarized as follows:
% 1) We present a novel method for achieving fast and accurate deformable tissue reconstruction. This method surpasses or matches the rendering quality of previous approaches, despite utilizing only monocular sequences. The reconstruction process time has been significantly reduced to a mere 3 minutes, surpassing previous methods by over 100-fold in terms of speed.
% 2) We propose an innovative and highly effective representation of surgical scenes that seamlessly integrates both static and dynamic fields. This integration enables rapid optimization and results in high-quality reconstructions.
% 3) We have developed an optimization algorithm specifically designed to adapt to implicit expressions. This algorithm further enhances the training and rendering speed, contributing to the overall efficiency and effectiveness of our approach.

\section{Related Work}
% \subsection{Related Works}
% Work has been done to reconstruct surgical scenes. Early SLAM-based methods[endo23,31,32] use depth estimation and fuse depth maps in 3D space. These methods either did not consider the existence of surgical tools or simplify the scenes to be static. Later work SuPer[endo 8] and EDSSR[endo 11] perform frameworks for single-view reconstruction with tool masking and depth estimation. However, they track deformation based on a sparse warp field, which become less effective when the deformations go beyond simple non-topological changes and become more complex. Recent work EndoNeRF[endonerf] uses NeRF with tool-guided ray casting, stereo depth-cueing ray marching and stereo depth-supervised optimization to achieve high-quality non-rigidity reconstruction. But the NeRF structure they use is significantly time and resource consuming. 
% There are many applications on Medical Imaging using NeRF[]. H. Li et al.[] explores the application of NeRF method in 3D ultrasound spine imaging, achieving clearer and more complete bone structure reconstructions while addressing challenges related to regularization and non-Lambertian effects. IOSNET[] introduces a Neural Field which maps points in high-resolution medical scans to occupancy values, providing continuous and memory-efficient segmentation maps, demonstrating advantages such as flexible resolution sampling, faster convergence, and reduced memory usage compared to voxel-based methods. ImplicitAtlas[] is an approach for precise and detailed shape completion in medical imaging, utilizing implicit, learned shape representations, template matching, and multi-scale features to address challenges posed by limited data and diverse object poses and scales.
\subsection{Surgical Scene Reconstruction}
% Various efforts have been made to reconstruct deformable tissues among surgical scenes. Some SLAM-based methods\cite{song2017dynamic, zhou2019real, zhou2021emdq} utilize depth estimation and fuse depth maps in 3D space to do reconstruction. However, these methods either overlook the presence of surgical tools or simplify the scenes by assuming them to be static. Subsequent advancements, \textit{e.g.} SuPer\cite{li2020super} and EDSSR\cite{edssr}, introduce frameworks for single-view reconstruction with tool masking and depth estimation. Nonetheless, these approaches employ deformation tracking based on a sparse warp field. 
% As a result, their effectiveness diminish when confronted with deformations that exceeded simple non-topological changes.
% In recent research, EndoNeRF\cite{endonerf} emerges as a promising solution, utilizing NeRF with tool-guided ray casting, stereo depth-cueing ray marching, and stereo depth-supervised optimization. This approach results in high-quality non-rigidity reconstruction. 
% However, EndoNeRF optimizes a full spacial field which end up makes it time and resource consuming. 
% To facilitate inter-operative use, greater efforts should be made to accelerate the process without compromising performance.
Numerous endeavors have been undertaken to reconstruct deformable tissues within surgical scenes. 

\subsubsection{Non-implicit Representations}
There have been numerous noteworthy non-implicit approaches in the realm of surgical scene reconstruction~\cite{schmidt2023tracking}. Earlier SLAM-based studies such as~\cite{song2017dynamic, zhou2019real, zhou2021emdq} leveraged depth estimation from stereo videos and fuse depth maps in 3D space for reconstruction. However, these methods either neglected the presence of surgical tools or oversimplified the scenes by presuming them to be static. Later advancements, such as SuPer~\cite{li2020super} and EDSSR~\cite{edssr}, proposed frameworks for stereo depth estimation with tool masking, and SurfelWarp~\cite{gao2019surfelwarp} performed single-view 3D deformable reconstruction. These approaches relied heavily on deformation tracking via a sparse warp field, which compromised their efficacy when encountering deformations that exceed simple non-topological changes.

\subsubsection{Novel Implicit Representations}
Implicit representations like NeRF~\cite{nerf} have made remarkable contributions to medical imaging.
In contrast to non-implicit representations, which encode discrete features or signal values directly, implicit representations use generator functions that associate input coordinates with their respective values within the input space~\cite{molaei2023implicit}.
Recently, EndoNeRF~\cite{endonerf} emerged as a promising solution. It utilized NeRF with tool-guided ray casting, stereo depth-cueing ray marching, and stereo depth-supervised optimization, yielding high-quality non-rigidity reconstruction. However, EndoNeRF optimized an entire spatial temporal field, resulting in significant time and resource consumption. 
Lerplane~\cite{lerplane} factorizes the scene into explicit 2D planes of static and dynamic fields to accelerate optimization, but the inference speed is insufficient to meet clinical demands. 
% cue Lerplane ?
Therefore, for effective inter-operative application, more intensive efforts must be dedicated towards speeding up the process without sacrificing the reconstruction performance.

% \subsubsection{Implicit Representation Acceleration}
% Implicit representation has shown impressive performance, while its optimization is relatively slow. Several explicit and hybrid methods have been developed to model static scenes and achieve speed improvements over NeRF, these methods have predominantly been applied to static scenes only. 

% The application of explicit methods to dynamic surgical scene reconstruction presents significant challenges. 
% While several explicit and hybrid methods have been developed to model static scenes and achieve speed improvements over NeRF, these methods have predominantly been applied to static scenes only. 
% When it comes to surgical scenes, there are two primary reasons why applying these methods becomes challenging.
% Firstly, encoding temporal information is crucial for accurately modeling surgical scenes. However, simply adding a temporal dimension to the explicit data structure can lead to a substantial increase in memory and computational requirements. This poses a practical limitation on the feasibility of using explicit methods for dynamic surgical scene reconstruction. 
% Secondly, dynamic surgical scene reconstruction faces limitations in terms of viewpoints, often providing only one view per timestep. In contrast, static scenes can leverage multi-view consistency to enhance regularization and improve reconstruction quality. This discrepancy in available viewpoints necessitates the sharing of information across disjoint timesteps to overcome the limitations and achieve better reconstruction quality.
% 
% \subsection{Explicit Representation in Medical Imaging}
% Traditional explicit representations usually directly encode the features or signal values in medical images\cite{molaei2023implicit}. 
% }

\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{figures/performance_a2}}
% \vspace{-0.5em}
\caption{Reconstruction results of deformable tissues. We show the deformable tissues reconstructed by Forplane among surgical procedures with the corresponding captured images in the lower-right corner.}
% \vspace{-2em}
\label{fig: our performance a}
\end{figure}

\subsection{Implicit Representations in Medical Imaging}
Implicit representations have yield significant contributions in other realms of medical imaging. Some methods leverage NeRF to perform visualization of medical images. For instance, Li et al.~\cite{li20213d} used NeRF to acquire 3D ultrasound reconstructed spine image volume to assess spine deformity. MedNeRF~\cite{corona2022mednerf} rendered CT projections given a few or even a single-view X-ray utilizing NeRF and GAN. NeAT~\cite{ruckert2022neat} used a hybrid explicit-implicit neural representation for tomographic image reconstruction, showing better quality than traditional methods. 
CoIL~\cite{sun2021coil} leveraged coordinate-based neural representations for estimating high-fidelity measurement fields in the context of sparse-view CT.
EndoNeRF~\cite{endonerf}, applied dynamic nerf~\cite{pumarola2021d} to perform deformable surgical scene reconstruction, showing promising performance on stereo 3D reconstruction of deformable tissues in robotic surgery. 
Some methods use implicit functions to do shape reconstruction. ImplicitAtlas~\cite{yang2022implicitatlas} proposed a data-efficient shape model based on templates for organ shape reconstruction and interpolation. 
Fang et al.~\cite{fang2022curvature} introduced a curvature-enhanced implicit function network for high-quality tooth model generation from CBCT images. 
Raju et al.~\cite{raju2022deep} presented deep implicit statistical shape models (DISSMs) for the 3D delineation of medical images.
For segmentation, IOSNET~\cite{khan2022implicit} used neural fields to create continuous segmentation maps which converge fast and are memory-efficient. 
TiAVox~\cite{zhou2023tiavox} used a time-aware attenuation voxel approach for sparse-view 4D DSA reconstruction. NeSVoR~\cite{10015091} modeled the underlying volume as a continuous function to perform slice-to-volume reconstruction. Reed et al. devised a reconstruction pipeline that utilizes implicit neural representations in conjunction with a novel parametric motion field warping technique to perform limited-view 4D-CT reconstruction of rapidly deforming scenes~\cite{reed2021dynamic}. Schmidt et al. introduced RING~\cite{schmidt2022recurrent} which estimates flow efficiently and KINFlow~\cite{schmidt2022fast} which enables a prior-free estimation of deformation, both using implicit neural representation and graph-based model.
% This bro probably is Schimidt himself. Should Cue him by name.
% applies GRAF\cite{schwarz2020graf}, a method using GAN to eliminate the necessity pose data, to

==> LaTeX/2_materias_and_method.tex <==
\section{Materials and Methods}

We focus on the task of efficiently reconstructing deformable tissues from both monocular and binocular endoscopy videos. Mathematically, we represent a surgical procedure as a 4D volume denoted by $\mathbf{V}_{4d}$, with dimensions $H\times W\times D \times T$. Here, $H, W, D$ represents the 3D space of the scene, and the $T$ represents the time dim, assumed to be orthogonal to the 3D space. Unlike previous methods that treat the surgical procedure as independent static 3D volumes per time step $\{\mathbf{V}_{3d}^{1}, \mathbf{V}_{3d}^{2},...,\mathbf{V}_{3d}^{T}\}$ or use a time-dependent displacement field $\mathbf{G}_{\boldsymbol\phi}$ to model the tissue deformations, we factorizes the 4D volumes into a static field $\mathbf{V}_{3d}^{s}$ and a dynamic field $\mathbf{V}_{3d}^{d}$ composed of 2D neural planes. This factorization significantly enhances convergence speed and improves the representational capacity.



In this section, we begin with reviewing the key techniques used in NeRF~\cite{nerf} and EndoNeRF~\cite{endonerf} (Sec. \ref{method: NeRF and EndoNeRF}). Subsequently, we introduce our novel and efficient orthogonal plane representation for surgical scenes (Sec. \ref{method: Neural Forplane Representation for Deformable Tissues}).
To reconstruct deformable tissues at any time step, we first employ a novel spatiotemporal sampling algorithm to identify high-priority tissue pixels and generate corresponding rays (Sec. \ref{method: Spatiotemporal Importance Sampling}). Next, we design one efficient ray marching method to generate discrete samples along the selected rays (Sec. \ref{method: efficient ray marching}). These samples are then used to retrieve corresponding features from orthogonal planes with linear interpolation.
The obtained features, along with the spatiotemporal information of the samples, are fed into a lightweight MLP that predicts radiance and density for each sample (Sec. \ref{method: Coordinate-Time Encoding}). Finally, we apply standard volume rendering to render the accumulated color and depth along the selected rays. 
To improve the spatiotemporal smoothness and decomposition, we design various regularization strategies on $\{\mathbf{V}_{3d}^{s}, \mathbf{V}_{3d}^{d}\}$ as well as the lightweight MLP (Sec. \ref{method: Optimization}).
% \repd{Finally, we present the adaptation of Forplane for monocular inputs (Sec. \ref{method: Forplane with Monocular Inputs}).}{
We present an optimization strategy for Forplane that diminishes its reliance on binocular depth so that it can work with monocular scopes (Sec. \ref{method: Forplane with Monocular Inputs}).
An illustration of the overall framework is presented in Fig.~\ref{fig: pipline}.
% It starts by using spatiotemporal importance sampling to identify high-priority tissue pixels and build corresponding rays (Sec.2.4).
% We then present several core components that improve optimization and accelerate inference, including the , , and the coordinate-time encoding method . Finally, we provide a detailed explanation of the loss functions used in our approach.

\begin{figure*}[ht]
% \vspace{-1.5em}
\centerline{\includegraphics[width=\textwidth]{LaTeX/figures/pipeline_v3.pdf}}
\caption{The rendering pipeline of Forplane. Forplane begins with spatiotemporal importance sampling (Sec.~\ref{method: Spatiotemporal Importance Sampling}), which assigns higher sampling probabilities to tissue pixels occluded by tools or with extensive motion. Following the selection of the pixel (ray) to be rendered, an efficient ray marching algorithm (Sec.~\ref{method: efficient ray marching}) samples spatial points along the ray near the tissue surface. The coordinates and time embeddings of sampled points are used to query their corresponding features from multi-scale orthogonal feature planes (\textit{e.g.}, $G_{XY}$) via linear interpolation (Sec.~\ref{method: Neural Forplane Representation for Deformable Tissues}). 
For simplicity, single-resolution planes exemplify these multi-scale neural planes. The features from different planes and scales are fused using element-wise multiplication in Forplane. To enhance temporal information, the fused plane features are concatenated with positional encoded coordinate and time embeddings (Sec.~\ref{method: Coordinate-Time Encoding} and Fig.~\ref{fig: MLP structure}), and then passed through a lightweight MLP~$\params$. Finally, a volume rendering scheme is applied to generate predicted color and depth values for each selected ray.}
\vspace{-1.5em}
\label{fig: pipline}
\end{figure*}

\subsection{NeRF and EndoNeRF}
\label{method: NeRF and EndoNeRF}
We provide a brief overview of the pipeline of NeRF~\cite{nerf} and EndoNeRF~\cite{endonerf}.
Given a set of posed images $\{\mathbf{I}_i\}_{i=1}^N$, NeRF represents a 3D scene using volume density and directional emitted radiance for each point in space with a coordinate-based neural network $\params$. To render one image $\mathbf I_{i}$, a ray casting process is performed for each pixel, where a ray $\mathbf{r}(t) = \mathbf{x}_{o} + t\mathbf{d}$ is projected through the camera pose. Here, $\mathbf{x}_o$ is the camera origin, $\mathbf{d}$ is the ray direction, and $t$ denotes the distance of a point along the ray from the origin. 
NeRF uses a positional encoding $\gamma(\cdot)$ to map the coordinates $\mathbf{x}$ and viewing direction $\dir$ into a higher dimensional space:
% \small
\begin{equation}
    \gamma(\mathbf{x})\!=\!\Big[ \sin(\mathbf{x}), \cos(\mathbf{x}), \ldots, \sin\!\big(2^{\numfrequencies-1} \mathbf{x}\big), \cos\!\big(2^{\numfrequencies-1} \mathbf{x}\big) \Big]^\transpose \,. \label{eq:posenc}
\end{equation}
\normalsize
The process of casting a ray through the scene and generating discrete samples along the ray is termed ray marching.
The color $\C(\ray)$ for a specific ray $\ray(t)$ is computed using volume rendering, which involves integrating the weighted volumetric radiance within the near and far bounds $\near$ and $\far$ of the ray:
% 
\begin{align}
\C(\ray) = \int_\near^\far \!\!\!
w(t)
\cdot
\underbrace{\radiance(\ray(t), \dir)}_\text{radiance}~dt
\label{eq:volume_render}
\end{align}
% 
The integration weights $w(t)$ for volume rendering are given by:
% 
\begin{align}
w(t) = \underbrace{\exp \left( -\int_{t_n}^{t} \density(\ray(s)) \, ds \right )}_\text{visibility of $\ray(t)$ from $\origin$} \:\: \cdot \!\!\!\! \underbrace{\density(\ray(t))\vphantom{\int_{t_n}^{t}}}_\text{density at $\ray(t)$}
\label{eq:weights}
\end{align}
% 
The training of $\params$ is supervised by an L2 photometric reconstruction loss.


EndoNeRF~\cite{endonerf} employs a canonical radiance field $F_\Theta(\mathbf{x}, \dir)$ and a time-dependent displacement field $G_\Phi(\mathbf{x}, \tau)$ to represent the surgical scene. The time-dependent displacement field maps the input space-time coordinates $(\mathbf{x}, \tau)$ to the displacement between point $\mathbf{x}$ at time step $\tau$ and its corresponding point in the canonical field.
For any given time step $\tau$, the radiance and density at $\mathbf{x}$ can be obtained by querying $F_\Theta(\mathbf{x} + G_\Phi(\mathbf{x}, \tau), \mathbf{d})$. 
EndoNeRF employs the same positional encoding algorithm to map the input coordinates and time step into Fourier features before feeding them into the networks.

% The color $\C(\ray)$ is computed by integrating the weighted volumetric radiance within the ray's near and far bounds $\near$ and $\far$:
% % 
% \begin{align}
% \C(\ray) = \int_\near^\far \!\!\!
% w(t)
% \cdot
% \!\!\underbrace{\radiance(t)}_\text{radiance} \!\! \, dt
% \label{eq:nerfcolor}
% \end{align}
% % 
% where $\ray(t)=\origin + t\mathbf{d}$ represents a ray with camera origin $\origin$ oriented as $\mathbf{d}$. The integration weights for volume rendering are given by:
% % 
% \begin{align}
% w(t) = \underbrace{\exp \left( -\int_{t_n}^{t} \density(s) \, ds \right)}_\text{visibility of $\ray(t)$ from $\origin$} \:\: \cdot \!\!\!\! \underbrace{\density(t)   \vphantom{\int_{t_n}^{t}}}_\text{density at $\ray(t)$}
% \label{eq:weights}
% \end{align}
% % 

% The intermediate features $\feature(t)$, volumetric density $\density(t)$, and view-dependent radiance fields $\radiance(t)$ are stored within the parameters $\params$ of fully connected neural networks:
% % 
% \begin{align}
% \feature(t) &= \feature(\ray(t); \params) : \real^3 \rightarrow \real^z 
% \label{eq:feature}
% \\
% \density(t) &= \density(\feature(t); \params) : \real^z \rightarrow \real^+ 
% \label{eq:density}
% \\
% \radiance(t) &= \radiance(\feature(t), \dir; \params) : \real^z \times \real^3 \rightarrow \real^3
% \label{eq:radiance}
% \end{align}
% % 
% The discretization of the integrals in \eqref{eq:nerfcolor} and \eqref{eq:weights} follows \cite{nerf}. As the scenes used in this work are observed at different distances, we employ the integrated positional encoding proposed in mip-NeRF for 3D points $\ray(t)$ and the original positional encoding for the viewing direction $\mathbf{d}$.

% NeRF has been introduced in 2019 as an approach to novel views rendering and scene 3D representation that is "contained" by a fully-connected, non-convolutional network. Basically, Neural Field stands for an MLP (Multi-Layer Perceptron) that has a 3D point (x, y, z) and camera viewing direction angles (α, β) as an input and outputs the volume density (e.g. zero if there is no object at this point) and view dependent radiance (rgb color) at the point from this viewing direction. NeRF uses the volume density and emitted radiance to characterize the scene structure and a traditional differentiable volume rendering to learn from the colors of the pixels in the input images.

\subsection{Fast Orthogonal Plane Representation}
\label{method: Neural Forplane Representation for Deformable Tissues}
The surgical procedure consists of a series of consecutive frames, each representing a separate scene. Notwithstanding the mutable nature of tissue transformations over time, a significant portion of the tissue structure demonstrates continuity across consecutive frames. Observing this, we propose a method that efficiently capitalizes on the time-invariant components of the tissue structures to construct a static field $\mathbf{V}_{3d}^{s}$. 
% \repd{To capture the time-aware deformations, a dynamic field $\mathbf{V}_{3d}^{d}$ is formulated.}{
The static field is designed to encapsulate invariant tissue structures across these frames, thereby enabling the reuse of static components without necessitating data duplication for each temporal step. This design significantly reduces the memory requirement by obviating the need to repeatedly store information pertaining to the static aspects of the scene in every frame. 
In addressing the time-aware deformations, we have formulated a dynamic field, denoted as $\mathbf{V}_{3d}^{d}$. This field is uniquely tasked with capturing the deviations from the static field. This focused approach allows the dynamic field to circumvent the need for a comprehensive reconstruction of the entire scene, thereby substantially diminishing the computational burden.
% \rep{The static field is designed to encapsulate invariant tissue structures across these frames, thereby enabling the reuse of static components without necessitating data duplication for each temporal step. This approach significantly reduces the memory requirement by obviating the need to repeatedly store information pertaining to the static aspects of the scene in every frame. Furthermore, the dynamic field is exclusively concerned with temporal variations, modeling only the changes relative to the static field. This targeted focus simplifies the construction of the dynamic field, as it requires capturing only the deviations from the static baseline, rather than reconstructing the entire scene.}
% \repd{Since the $\mathbf{V}_{3d}^{s}$ is ``static'', }{
To build the static field, 
% }
we adopt the orthogonal space planes (\textit{i.e.}, $G_{\textit{XY}}$, $G_{\textit{YZ}}$ and $G_{\textit{XZ}}$) to represent the static components among the surgical procedure. The use of orthogonal space planes has been proven effective and compact in various static scene reconstruction methods~\cite{tensorf, instantngp}.
%
As for the $\mathbf{V}_{3d}^{d}$, it is designed to capture the time-dependent appearance. Since the time dimension is orthogonal to the 3D space, it is natural to employ space-time planes (\textit{i.e.}, $G_{\textit{TX}}$, $G_{\textit{TY}}$ and $G_{\textit{TZ}}$) to represent the dynamic field. 
%
Each space plane has dimensions of $N \times N \times D$, and each space-time plane has dimensions of $N \times M \times D$, where $N$ and $M$ denote the spatial and temporal resolutions, respectively, and $D$ represents the size of the feature stored within the plane.

% introduce the main pipeline
To render one tissue pixel $p_{ij}$ in a specific time step $\tau$, we first cast a ray $\mathbf{r}(t)$ from $\mathbf{x}_o$ to the pixel. We then sample spatial-temporal points along the ray, obtaining their 4D coordinates. We acquire a feature vector for a point $\mathbf{P}(x, y, z, \tau)$ by projecting it onto each plane and using bi-linear interpolation $\mathcal{B}$ to query features from the six feature planes:
\begin{align}
    \mathbf{v}(x,y,z,\tau) = & \mathcal{B}(G_{\textit{XY}}, x, y) \odot \mathcal{B}(G_{\textit{YZ}}, y, z) \notag \\  & \cdots \mathcal{B}(G_{\textit{YT}}, y, \tau) \odot \mathcal{B}(G_{\textit{ZT}}, z, \tau), \label{eq:interpolate}
\end{align}
where $\odot$ represents element-wise multiplication, inspired by~\cite{fridovich2022plenoxels, cao2023hexplane, fridovich2023k}. The fused feature vector $\mathbf{v}$ is then passed to a tiny MLP $\params$, which predicts the color $\radiance(\ray(t), \dir)$ and density $\sigma(\ray(t))$ of the point. Finally, we leverage the Eq.~\ref{eq:volume_render} to get the predicted color $\C$. Inspired by the hybrid representation of static fields~\cite{instantngp}, we build $\{\mathbf{V}_{3d}^{s}, \mathbf{V}_{3d}^{d}\}$ with multi-resolution planes. 
% $\textit{e.g.}$, the feature plane $G_{\textit{XY}}$ is built with three resolution, with $N = 128, 256~\text{and}~512$.

% Forplane factorizes the continuous dynamic space into a time-independent static field and a time-varying dynamic field, modeled using multi-resolution discrete feature planes. 
The factorization of surgical procedure brings three main benefits: 
1) Significant acceleration: Existing methods for reconstructing surgical procedures using pure implicit representations require traversing all possible positions in space-time, resulting in high computational and time complexity. In contrast, querying a Forplane is fast and efficient, involving only several bilinear interpolations among feature planes and a vector matrix product. This reduces the computational cost from O$(N^4)$ to O$(N^2)$. Moreover, this factorization lightens the burden on the MLP, enabling the use of lighter MLP architectures, 
% \repd{which leads to substantial acceleration in both the optimization and inference processes. }{
comprising just 2 fully connected layers, each with 64 channels. In contrast, EndoNeRF~\cite{endonerf} employs a complex MLP structure, processing the positional encoding of the input location $\gamma(x)$ through 8 fully connected ReLU layers, each with 256 channels.
2) Sharing learned scene priors: The static field in Forplane facilitates information sharing across different time steps, improving reconstruction performance by incorporating learned scene priors.
3) Modeling arbitrary deformation: Compared with displacement field used by~\cite{du2021neural, li2021neural, park2021nerfies, tineuvox, endonerf} which struggles with changes in scene topology, the dynamic field can easily model complex tissue deformations, allowing for more accurate reconstruction in surgical scenes.

% claim the advantage
% Forplane factorizes the continuous dynamic space into a time-independent static field and a time-varying dynamic field, both of which are modeled through multi-resolution discrete feature planes. This factorization offers three main benefits:
% 1) Significant acceleration: Existing methods for reconstructing surgical procedures using pure implicit representations require traversing all possible positions in space-time, resulting in high computational and time complexity. In contrast, querying a Forplane is fast and efficient, involving only several bilinear interpolations among feature planes and a vector matrix product. This reduces the computational cost from O$(N^4)$ to O$(N^2)$.
% Furthermore, in pure implicit representations, MLP is responsible for establishing the mapping from spatiotemporal coordinates to radiance and density values. In contrast, in Forplane, neural planes are employed to establish the mapping between coordinates and features. As a result, the MLP is only tasked with mapping features to radiance and density, significantly reducing the computational burden on the MLP itself. This reduction in complexity enables the use of lighter MLP architectures, which leads to substantial acceleration in both the optimization and inference processes. 
% 2) Sharing learned scene priors. Dynamic surgical scene reconstruction faces limitations in terms of viewpoints, often providing only several views on specific tissue. The existence of the static field in Forplane encourages the neural network to share information across different time steps, facilitating the utilization of learned scene priors and leading to improved reconstruction performance. This incorporation of multi-view consistency enhances the accuracy and robustness of the reconstructed surgical scenes.
% 3) Modeling arbitrary deformation. Previous methods that employ individual MLPs to represent deformation and canonical fields assume the absence of topology changes, which does not hold in surgical procedures where tissues undergo non-rigid deformation most of the time. Forplane addresses this limitation by using a time-relevant field instead of coordinate mapping to model any type of deformation. This property allows for better modeling of complex tissue deformations, enabling more accurate reconstruction of deformable tissues in surgical scenes.
% Methods that employ individual MLPs to represent a deformation field and a canonical field hold on the assumption that there are no topology changes, which does not hold in the surgical procedure since the tissues perform non-rigid deformation most of the time. Our dynamic field ease the assumption, using a time-relevant field rather than coordinate mapping to model any type of deformation. This property helps us to model the complex tissue deformation better.


\subsection{Spatiotemporal Importance Sampling}
\label{method: Spatiotemporal Importance Sampling}
Tool occlusion during robotic surgery poses significant challenges in accurately reconstructing occluded tissues due to their infrequent representation in the training set. As a result, different pixels encounter varying levels of difficulty in the learning process, exacerbating the complexity of tissue reconstruction. Furthermore, the presence of stationary tissues over time leads to repeated training on these pixels, yielding minimal impact on convergence and diminishing overall efficiency \cite{yang2023nerfvs}. To tackle these challenges, we devise a novel spatiotemporal importance sampling strategy. 
It prioritizes tissue pixels that have been occluded by tools or exhibit extensive motion ranges by assigning them higher sampling probabilities.

In particular, we utilize binary masks $\{\boldsymbol{M}_i\}_{i=1}^T$ and temporal differences among frames to generate sampling weight maps $\{\boldsymbol{W}_i \}_{i=1}^T$. These weight maps represent the sampling probabilities for each pixel/ray, drawing inspiration from EndoNeRF~\cite{endonerf}.
One sampling weight map $\boldsymbol{W}_i$ can be determined by:
\begin{align}
    \boldsymbol{W}_i &= \min(\max_{\substack{i-n<j\\<i+n}} (\|\ \boldsymbol{I}_i\odot\boldsymbol{M}_i - \boldsymbol{I}_j\odot\boldsymbol{M}_j \|_1)/3, \alpha)\odot\bm{\mathit\Omega}_i, \notag \\ 
    \bm{\mathit\Omega}_i &= \beta(T\boldsymbol{M}_i/ {\sum\limits_{i=1}^T\boldsymbol{M}_i}),
\end{align}
where $\alpha$ is a lower-bound to avoid zero weight among unchanged pixels, $\bm{\mathit\Omega}_i$ specifies higher importance scaling for those tissue areas with higher occlusion frequencies, and $\beta$ is a hyper-parameter for balancing augmentation among frequently occluded areas and time-variant areas. 
By unitizing spatiotemporal importance sampling, Forplane concentrates on tissue areas and speeds up training, improving the rendering quality of occluded areas and prioritizing tissue areas with higher occlusion frequencies and temporal variability. 


\subsection{Efficient Ray Marching}
\label{method: efficient ray marching}
The process of volume rendering greatly benefits from the precise sampling of spatiotemporal points, particularly around tissue regions.
% \redstrike{Although the sample-net introduced in [37] delivers improved precision near the surface, it also necessitates extensive point sampling throughout the whole pipeline, which substantially slows down inference speed.}
Both EndoNeRF \cite{endonerf} and the original version Lerplane \cite{lerplane} introduce specialized sampling schemes to enhance point accuracy. EndoNeRF's approach involves a stereo depth-cueing ray marching module that utilizes stereo depth data to guide point sampling near tissue surfaces. However, this method is limited in scenarios lacking accurate stereo depth information. Conversely, our original version Lerplane \cite{lerplane} employs a sample-net for surface-focused sampling. While effective, this approach requires extensive sampling across the pipeline, leading to reduced inference speeds.

To address this issue, we design an indicator grid that directs the Forplane's focus towards the tissue surface. This method is inspired by the grid representation method~\cite{fridovich2022plenoxels, nerfacc, instantngp, tensorf} used in static scene reconstruction, and it serves to optimize ray marching. The indicator grid functions as a binary map which is cached and updated throughout the training process, signifying empty areas. This low cost grid allows for the early termination of the marching process, based on the transmittance along the ray.

% As illustrated in eq.~\ref{eq:volume_render}, the pixel color rendered is the weighted sum of the radiance along the ray. We query the radiance field for the corresponding radiance and density of a sample point. The existing coarse-to-fine sample strategy for spatial temporal points is time-consuming, hence our modification. By utilizing the pre-learned scene context distribution, we can disregard points that minimally contribute to rendering results and sample points near the surface with greater precision. This change enhances the rendering quality, especially among deformable tissues.

% The technique involves maintaining two identical resolution occupancy grids, where each grid cell houses occupancy encoded as a single bit, arranged in Morton (z-curve) order to enable memory-coherent traversal by a digital differential analyzer during ray marching. If the cell's bit is low, the sample is omitted from the step size of the previous section.

For optimization efficiency, we integrate the indicator grid update with Forplane's standard training. We start with the assumption that all space is dense, and the indicator grid is fully occupied. As we introduce a series of spatial temporal points to Forplane, we pass a small batch sampled from them to the tiny MLP $\params$ to obtain the corresponding density, updating the indicator grid accordingly.
Initially, the optimization process is somewhat slow. However, after several iterations, the indicator grid becomes capable of identifying the density distribution within the 4D volume. This capability significantly reduces the need for unnecessary point sampling, which in turn greatly enhances the speed of training.

% Although the optimization speed is initially slow, after several iterations, the indicator grid can identify the actual distribution and significantly reduce unnecessary point sampling.

Our low cost indicator grid allows for efficient ray marching during both the optimization and inference stage. Leveraging the pre-learned scene context distribution allows us to ignore points with minimal contribution to rendering results and sample points near the surface more accurately. This change improves rendering quality, especially for deformable tissues. Compared to the original version~\cite{lerplane}, our novel efficient ray marching enables faster training and substantially improves rendering speed, approximately 5 times faster (\textbf{\textit{1.73~fps}} vs. \textbf{\textit{0.38~fps}}), representing a significant advancement for intraoperative use.

\subsection{Coordinate-Time Encoding}
\label{method: Coordinate-Time Encoding}
In Section \ref{method: NeRF and EndoNeRF}, it is illustrated that previous methods utilize a positional encoding function $\gamma(\cdot)$ to map coordinates and viewing directions into a higher-dimensional space. The positional encoding of the viewing direction is exploited to capture the view-dependent appearance, which operates on the assumption of a stationary environmental light source. However, this modeling method proves ineffective within the context of an in vivo sequence. The primary reason for this inefficacy is the dynamic nature of the light source, which moves in conjunction with the camera, bound by specific constraints. Consequently, the modeling of the view-dependent appearance becomes arbitrary, which leads to inaccurate scene reconstruction.

\begin{figure}[t]
\centerline{\includegraphics[width=0.8\columnwidth]{figures/MLP}}
% \vspace{-0.5em}
\caption{The procedure of Coordinate-Time Encoding. We pass positional encoded coordinate and time embeddings to enhance the temporal information. The tiny MLP ($\params$) consists of the sigma net $\theta_\sigma$ and the color net $\theta_{\mathbf c}$. The blue and yellow boxes denote MLP layers with and without ReLU activation.}
\label{fig: MLP structure}
% \vspace{-1.5em}
\end{figure}

Rather than inputting positionally-encoded viewing information, we propose an enhancement on spatiotemporal information, as shown in Fig.~\ref{fig: MLP structure}. This enhancement involves concatenating interpolated features in Eq.~\ref{eq:interpolate} with positionally encoded coordinates and temporal embeddings. This new approach ensures a more precise representation of the scene and a more accurate reflection of the dynamic conditions inherent in an in vivo sequence.
In this work, we use one-blob~\cite{oneblob} encoding separately on each of the four coordinate values. 
The formulation of one-blob encoding is:
% \begin{equation}
% \mathbf{b}(\mathbf{x}) = \frac{1}{|\Psi(\mathbf{x})|} \sum_{\mathbf{y} \in \Psi(\mathbf{x})} \mathbf{f}(\mathbf{y}),
% \label{one-blob_encode}
% \end{equation}
% \textcolor{red}{encoding should be inline with input and output}
% where $\mathbf{x}$ is the vector to be encoded, $\Psi(\mathbf{x})$ is a local region surrounding the vector, $|\Psi(\mathbf{x})|$ is the number of vectors in the region, and $\mathbf{f}(\mathbf{y})$ is a vector of features extracted from a vector $\mathbf{y}$ in the region.

\begin{equation}
    \mathbf{b}(s) = g_{s, \xi^2}(\frac{i-0.5}{k}), i = 1, 2, 3\dots k,
\end{equation}
where $g_{s, \xi^2}$ is a Gaussian kernel with mean value $s$ and variance $\xi^2$. 
The encoding function maps $s \in \mathbb{R}$ into a higher dimensional space $\mathbb{R}^k$. 
% here s is a scalar within a vector. we set nbins = 4, $\sigma = \frac{1}{nbins}$. $g_{s, \sigma^2}$ is a Gaussian function with paras $(\mu, \sigma)$ = $(s, \sigma)$ 
The encoding along with the fused features $\mathbf{v}$ from feature planes is input to the MLP $\params$, which predicts $\sigma$ and $\mathbf c$ of each point. Then we utilize Eq.~\ref{eq:volume_render} to render the expected color $\hat{\boldsymbol{C}}$ and depth $\hat{\boldsymbol{D}}$ of one specific ray. 

% The whole rendering procedure is described in Algorithm 1. 
% We starts from a specific ray $\mathbf r(t) = (\mathbf x_o +t\mathbf d )$ which is decided by spatiotemporal importance sampling. 
% Then we uniformly sample points across the field, represented by $\boldsymbol{\mathcal P}u$. 
% These points are passed to the indicator grid $\mathbf G{o}$ to to get samples $\boldsymbol{\mathcal P}$ that distributes around the surface. For each sample point $\mathbf P(x, y, z, \tau)$ in the new sampled set $\boldsymbol{\mathcal P}$, the algorithm performs a series of operations:
% It initializes a vector $\mathbf v(x, y, z, \tau)$.
% For each pair of fields and their associated dimensions (e.g., $(xy, xz, x\tau, yz, y\tau, z\tau)$), it performs bi-linear interpolation using function $\mathcal B$ on the respective grid $G$ and updates the vector $\mathbf v$.
% The algorithm concatenates the bi-linear interpolation results with basis functions $\mathbf b(x, y, z, \tau)$, forming a feature set. 
% This feature set is then processed by the tiny MLP $\boldsymbol\theta$, which outputs color $\mathbf c_i$ and density $\mathbf \sigma_i$ for each point.
% Finally, we leverage volume rendering (Eq.~\ref{eq:volume_render}) to compute the expected color $\hat{\boldsymbol C}$ and depth $\hat{\boldsymbol D}$ of the ray.

{
{
\begin{algorithm}[t]
\small
\caption{The Rendering Procedure\label{algo:viewcoveragealgo}}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwComment{Comment}{/* }{ */}
\SetKwInOut{Define}{Functions}
\Input{A specific ray $\mathbf r(t) = (\mathbf x_o +t\mathbf d )$, 4 levels of the static field and the dynamic field $\{\mathbf{V}_{3d}^{s}$, $\mathbf{V}_{3d}^{d}\}^4$, the indicator grid $\mathbf G_{o}$ and the tiny MLP $\boldsymbol\theta$}
\Output{The expected color $\hat{\boldsymbol{C}}$ and depth $\hat{\boldsymbol{D}}$ of $\mathbf r(t)$}
$\boldsymbol{\mathcal P}_u \leftarrow $Uniformly sampled points \\
$\boldsymbol{\mathcal P}\leftarrow \mathbf G_o(\boldsymbol{\mathcal P}_u)$ to get sample points around the surface\\
\For{$\mathbf P(x, y, z, \tau)$ in $\boldsymbol{\mathcal P}$}
{   
    $\mathbf v(x, y, z, \tau) \leftarrow \mathbf 1$ to initialize\\
    % \For{$G, (i, j))$ in $\operatorname{zip}(\{\mathbf V^s_{3d}, \mathbf V^d_{3d}\}^4, \{(x, y), (x, z), (x, \tau), (y, z), (y, \tau), (z, \tau)\})$}
    \For{$G, ij$ in $\operatorname{zip}(\{\mathbf V^s_{3d}, \mathbf V^d_{3d}\}^4, \{(xy, xz, x\tau, yz, y\tau, z\tau\})$}
    {
        $\mathbf v(x, y, z, \tau) \leftarrow \mathbf v(x, y, z, \tau) \odot \mathcal B(G, i, j)$,\\
        ~$\mathcal B$ \text{is the bi-linear interpolation on $G$}
    }
    $\text{features} \leftarrow \operatorname{concat}(\mathbf b(x, y, z, \tau), \mathbf v(x, y, z, \tau))$ \\
    $(\mathbf c_i, \mathbf \sigma_i) \leftarrow \boldsymbol\theta (\text{features})$
}
$\hat{\boldsymbol C} \leftarrow \int_{t_n}^{t_f} w(t) \cdot \radiance(\mathbf r(t), \mathbf d)~dt$, $\hat{\boldsymbol D} \leftarrow \int_{t_n}^{t_f} w(t)\cdot t~dt$, $w(t) = \exp \left( -\int_{t_n}^{t} \density(\ray(s) \, ds )\right) \density(\ray(t))\vphantom{\int_{t_n}^{t}}$\\
return $\hat{\boldsymbol C}, \hat{\boldsymbol D}$;
\end{algorithm}
\label{algo: rendering}
}
}

Algorithm 1 demonstrates our rendering procedure, starting with a ray $\mathbf r(t) = (\mathbf x_o +t\mathbf d )$ selected through spatiotemporal importance sampling. We uniformly sample points along $\mathbf r(t)$, forming a point-set $\boldsymbol{\mathcal P}u$. This set is passed to the indicator grid $\mathbf G{o}$ to obtain $\boldsymbol{\mathcal P}$, which is distributed around the target tissue. 
We initialize each point in $\boldsymbol{\mathcal P}$ with 1 (the multiplicative identity).
Subsequently, we apply bi-linear interpolation to extract features from different feature planes (\textit{e.g.}, $G_{XY}$) using corresponding dimension (\textit{e.g.}, $xy$) and update $\mathbf v$ with element-wise multiplication accordingly. These features, combined with positional encoded coordinate and time embeddings $\mathbf b(x, y, z, \tau)$, are processed by the tiny MLP $\boldsymbol\theta$ to yield color $\mathbf c_i$ and density $\mathbf \sigma_i$. Finally, volume rendering (Eq.~\ref{eq:volume_render}) is applied to calculate the color $\hat{\boldsymbol C}$ and depth $\hat{\boldsymbol D}$ of $\mathbf r(t)$ by integrating radiance and density along the ray.


\subsection{Optimization}
\label{method: Optimization}
Reconstructing surgical procedures rapidly and accurately presents significant challenges due to the inherent uncertainty and limited information. To expedite the optimization of the tiny MLP and orthogonal planes, we incorporate not only supervision from color and depth but also spatiotemporal continuity constraints. Furthermore, we devise a disentangle loss to aid in the disentanglement of static and dynamic fields. 
% To mitigate reliance on binocular depth, we propose a set of optimization algorithms leveraging monocular depth estimation. 
The following sections comprehensively demonstrate the utilization of the employed loss function in our approach.
\subsubsection{Color Loss}
We utilize captured images to optimize both the tiny MLP $\params$ and the neural plane representation $\boldsymbol{\phi} = \{\mathbf{V}_{3d}^s, \mathbf{V}_{3d}^d\}$ concurrently. We define the color loss in the following manner:
\begin{equation}
\loss{rgb}(\params, \boldsymbol{\phi}) = \sum_{i} \expect_{\ray \sim \boldsymbol\image_i}
\left[
\norm{\C(\ray) - \boldsymbol{C}^\gt_i(\ray)}_2^2
\right],
\label{eq:rgb loss}
\end{equation}
where $\boldsymbol{C}^\gt_i(\ray)$ represents the ground truth color of the ray $\ray$ passing through a pixel in image $I_{i}$.

\subsubsection{Depth Loss}
Following the methodology laid out in EndoNeRF~\cite{endonerf}, we also employ depth information generated by stereo matching to assist in the optimization of the neural scene. We define the depth loss as follows:
\begin{equation}
\loss{depth}(\params, \boldsymbol{\phi}) = \sum_{i} \expect_{\ray \sim \boldsymbol D_i}
\left[
H_{\delta}\left(\hat{\boldsymbol{D}}(\ray) - \boldsymbol{D}^\gt_i(\ray)\right)
\right],
\label{eq:gt depth loss}
\end{equation}
where the $H_{\delta}$ represent standard huber loss and $\boldsymbol{D}^\gt_i(\ray)$ represents the depth predicted by the stereo matching algorithm of the ray $\ray$.

\subsubsection{Total Variation Loss}
Inspired by \cite{fridovich2022plenoxels} and \cite{niemeyer2022regnerf}, we also leverage the total variation regularization to help optimizing our method. Specifically, the $\mathcal{L}_{TV}$ is defined as:
\begin{equation}
    \mathcal L_{TV} = \displaystyle\sum_{G \in \mathbf{V}_{3d}^{s}} \displaystyle\sum_{g \in G} \left\| \Delta^2_h (G, g) + \Delta^2_w (G, g) \right\|,
\end{equation}
where $\mathbf{V}_{3d}^{s} = \{G_{XY}, G_{YZ}, G_{XZ}\}$ denotes all space planes in Forplane. $\Delta^2_h (G, g)$ represents the squared difference between the $g$th value in plane $G:=(i, j)$ and the $g$th value in plane $G:=(i+1, j)$ normalized by the resolution, and analogously for $\Delta^2_w (G, g)$. 

% \textcolor{red}{here, g need reformulate}
% $g$ is one of the elements in $G$. $\Delta^2_h (G, g)$ represents the difference along the first axis on element $g$ and analogously for $\Delta^2_w (G, g)$.

\subsubsection{Time Smoothness Loss}
To robustly reconstruct deformable tissue under limited view , we further incorporate time smoothness regularization for all space-time planes. This time smoothness term, akin to total variation loss, aims to ensure similarity between adjacent frames. The formulation is as follows:
\begin{equation}
    \mathcal L_{TS} = \displaystyle\sum_{G \in \mathbf{V}_{3d}^{d}}  \displaystyle\sum_{g \in G}\left\|\Delta_t^2 (G, g)\right\|,
\end{equation}
where $\mathbf{V}_{3d}^{d} = \{G_{XT}, G_{YT}, G_{ZT}\}$ is the set of the space-time planes in Forplane. $\Delta^2_x (G, g)$ represents the difference along the time axis.

% where $N_g$ is the number of elements in the $g th$ level of the grid.

\subsubsection{Disentangle Loss}
\label{Disentangle Loss}
As discussed in Sec.~\ref{sec:introduction}, surgical scenes pose a unique challenge due to the limited viewpoints they offer. This limitation necessitates sharing information across non-sequential timesteps to enhance the reconstruction quality. Our methodology employs a static-dynamic structure to model these surgical scenes. However, this structure creates an ambiguity for the model in discerning which areas should be modeled in the static field and which ones in the dynamic field.
To tackle this issue, we commence by initializing the values in $\mathbf{V}_{3d}^{d}$ to 1, which do not influence the features in $\mathbf{V}_{3d}^{s}$ during element-wise multiplication. 
% This is crucial because the number 1 serves as the multiplicative identity during the interpolation process as outlined in eq.~\ref{eq:interpolate}.
Subsequently, we optimize the model using a specialized disentangle loss function.
The $\mathcal{L}_{DE}$ is described as follows:
\begin{equation}
    \mathcal{L}_{DE} = \displaystyle\sum_{G \in \mathbf{V}_{3d}^{d}} \displaystyle\sum_{g \in G}\left\|1-g\right\|.
\label{eq: disentangle loss}
\end{equation}
With this regularization, the features of the space-time planes will tend to remain the initial value. This strategy allows us to maximize the use of the static field in modeling static scenes while also appropriately accounting for dynamic elements.

% \subsubsection{Monocular Loss}
% \begin{equation}
%     \mathcal L_{Mono} = \left\| \hat D\eta+\epsilon^* - D_{gt}\right\|_2^2
% \end{equation}
% Where $\hat D$ is the depth estimated by the planes, $D_{gt}$ is the ground truth depth. $\eta, \epsilon^*$ are parameters of the least square method given by $\eta = (\hat D^T \hat D)^{-1} \hat D^T D_{gt}$ and $\epsilon = D_{gt} - \hat D\eta$.

\textbf{Total Loss}: The total loss optimized during each iteration is defined as:
\begin{align}
    \mathcal{L}_{total}(\params, \mathbf{\boldsymbol{\phi}}) =& \mathcal{L}_{rgb} + \lambda_{d} \mathcal{L}_{D} + \lambda_{tv} \mathcal{L}_{TV} \notag \\  
    &+ \lambda_{ts} \mathcal{L}_{TS} + \lambda_{de} \mathcal{L}_{DE}.
\end{align}
In all experiments conducted, we set the parameters $\lambda_d = 1, \lambda_{tv} = 0.001, \lambda_{ts} = 0.05, \lambda_{de} = 0.001$, unless otherwise specified in the experimental design.
% where $\lambda_{*}$ represents the hyper-parameter employed to balance different losses.

% \subsection{Implement Details}
% All experiments were conducted on an Ubuntu 20.04 system equipped with dual Intel Xeon CPU E5-2697 processors and 4 NVIDIA GeForce RTX 3090 GPUs. Our Forplane is implemented via pure pytorch~\cite{NEURIPS2019_9015}.
% To handle view-limited endoscopy videos, the scene was transformed into normalized device coordinates (NDC) for ray casting within this NDC space. The video duration was standardized to the range of $[-1, 1]$ based on frame numbers. Efficient ray marching employed occupancy grids with a resolution of 64, filtering out points with density below 1e-4 to reduce computational overhead. Spatiotemporal information was encoded using the Oneblob encoding method. The complete model consisted of four spatial resolution levels: 64, 128, 256, and 512 dimensions. Key hyperparameters included feature planes with $D=32$, spatiotemporal importance sampling with $j=25$, Oneblob encoding dimensionality of $\xi=16$, and the depth loss parameter of $\delta=0.05$. These hyperparameters were consistently applied across all experiments, unless otherwise specified. Optimization utilized the Adam optimizer with standard parameters. Each training iteration randomly sampled a batch of 2048 rays from the comprehensive dataset. The initial learning rate was set to 0.01, accompanied by a cosine schedule and a warming-up phase of 512 iterations. Training was performed for both 9k and 32k iterations, with training durations approximately lasting 3 and 10 minutes, respectively.


% \smallskip\noindent
% \begin{small}
% \begin{tabular}{l}
% \verb+\+\texttt{documentclass[journal,twoside,web]\{ieeecolor\}}\\
% \verb+\+\texttt{usepackage\{\textit{Journal\_Name}\}}
% \end{tabular}
% \end{small}

\subsection{Forplane with Monocular Inputs}
\label{method: Forplane with Monocular Inputs}
In endoscopic procedures, monocular cameras are commonly used due to their compact size, despite some laparoscopes having stereo scope cameras. 
% \repd{To broaden the applicability of Forplane and reduce the reliance on binocular depth, we incorporate data-driven monocular geometric cues. In this paper,}{
In the context of these scopes, the reliance on stereo depth in the original method \cite{lerplane} poses limitations. To address this, our enhanced version introduces an innovative optimization method tailored for monocular scopes. This method integrates data-driven monocular geometric cues into our training pipeline more effectively. In particular,
% }
we employ an off-the-shelf monocular depth predictor~\cite{bhat2023zoedepth} to generate a depth map $\{\bar{\boldsymbol{D}}_i\}_{i=1}^N$ for each input RGB image $\{\boldsymbol{I}_i\}_{i=1}^N$. Note that estimating absolute scale in surgical scenes is challenging; hence, depth should be treated as a relative cue. Yet, this relative depth information is beneficial even over larger distances in the image.

% Most endoscopic procedures, including colonoscopies, predominantly employ monocular cameras due to their compact size, despite a subset of laparoscopes being equipped with stereo scope cameras. In order to broaden the applicability of Forplane and alleviate data requirements on ground truth depth, we incorporate data-driven monocular geometric cues as a key component in our approach for surgical scene modeling. Such geometric cues have consistently showcased their effectiveness in bolstering the stability of optimization, particularly in challenging scenarios.

% A commonly used monocular geometric cue is a depth map, which can be conveniently obtained via an off-the-shelf monocular depth predictor. In our method, we employ a pre-trained monocular depth estimator to generate a depth map $\{\bar{\boldsymbol{D}}_i\}_{i=1}^N$ for each input RGB image $\{\boldsymbol{I}_i\}_{i=1}^N$. It should be noted that estimating absolute scale in surgical scenes is challenging; hence, depth should be treated as a relative cue. Yet, this relative depth information is beneficial even over larger distances in the image.

In light of these considerations, we introduce a monocular depth loss $\mathcal{L}_{Mono}$ to enforce consistency between the estimated depth $\hat{\boldsymbol{D}}(\ray)$ and the predicted monocular depth $\bar{\boldsymbol{D}}(\ray)$:
\begin{align}
    \mathcal L_{Mono}(\params, \boldsymbol{\phi}) &= \sum_{i} \expect_{\ray \sim \bar{\boldsymbol{D}}_i}
\left\|(\eta \hat{\boldsymbol{D}}(\mathbf{r})+\epsilon)-\bar{\boldsymbol{D}}(\mathbf{r})\right\|^{2}, \notag \\
\text{where}~\eta &= \left({\hat{\boldsymbol{D}}(\ray)}^T \hat{\boldsymbol{D}}(\ray)\right)^{-1} {\hat{\boldsymbol{D}}(\ray)}^T \bar{\boldsymbol{D}}(\ray), \notag \\
\epsilon &= \bar{\boldsymbol{D}}(\ray) - \eta \hat{\boldsymbol{D}}(\ray).
\end{align}
The $\eta$ and $\epsilon$ are the closed-form solution obtained via a least-squares criterion.
These parameters are calculated separately for each batch, as the predicted depth maps can vary in scale and shift across different batches. For monocular endoscopic sequences, we replace $\mathcal{L}_{D}$ with $\mathcal{L}_{Mono}$ during training. 
% For monocular endoscopic sequences, we replace $\mathcal{L}_{D}$ with $\mathcal{L}_{Mono}$ in the above loss function.

==> LaTeX/3_exps.tex <==
\section{experiments}
\subsection{Datasets}
\subsubsection{EndoNeRF Dataset} 
We assess the performance of Forplane using the EndoNeRF dataset~\cite{endonerf}. This dataset is a collection of typical robotic surgery videos captured via stereo cameras from a single viewpoint during in-house DaVinci robotic prostatectomy procedures. Specifically designed to capture challenging surgical scenarios characterized by non-rigid deformation and tool occlusion, the dataset serves as an ideal platform for evaluation. 
The dataset is composed of six video clips (in total 807 frames) with resolution of 512$\times$640 and lasting 4-8 seconds at a frame rate of 15 frames per second. The surgical challenges depicted in each case varies. Specifically, two cases (\textit{thin structure}, \textit{traction}) show traction on thin structures. Another two cases (\textit{pushing tissues}, \textit{pulling tissues}) depict significant manipulation of tissue through pushing or pulling. The final two cases (\textit{cutting twice}, \textit{tearing tissues}) capture the process of tissue cutting. 
These scenarios effectively illustrate the challenges inherent in managing soft tissue deformation and tool occlusion during surgery. 
% In line with the evaluation protocol of EndoNeRF, our method demonstrates superior acceleration and high-fidelity rendering performance amidst these complex surgical scenes.

\subsubsection{Hamlyn Dataset}
We evaluate our method using the public Hamlyn dataset~\cite{hamlyn1,hamlyn2}, which includes both phantom heart and in-vivo sequences captured during da Vinci surgical robot procedures. The rectified images, stereo depth, and camera calibration information are from \cite{endo-depth-and-motion}. 
To generate instrument masks, we utilize the widely-used vision foundation model, Segment Anything~\cite{kirillov2023segment}, which enables semi-automatic segmentation of surgical instruments.

The Hamlyn dataset presents a rigorous evaluation scenario as it contains sequences that depict intracorporeal scenes with various challenges, such as weak textures, deformations, reflections, surgical tool occlusion, and illumination variations. We select seven specific sequences from the Hamlyn dataset (Sequence: rectified01, rectified06, rectified08, and rectified09), each comprising 301 frames with a resolution of 480 $\times$ 640. These sequences span approximately 10 seconds and feature scenarios involving surgical tool occlusion, extensive tissue mobilization, large deformations, and even internal tissue exposure. To train and evaluate our method effectively, we divide the frames of each sequence into two sets: a training set of 151 frames and an evaluation set comprising the remaining frames. This division allows us to train our method adequately while providing a robust set for evaluation.
% We further encompass an evaluation of our method utilizing the public Hamlyn dataset. This dataset is composed of a phantom heart and in-vivo sequences that include exploratory trajectories executed with a da Vinci surgical robot. The data we analyze includes rectified images, stereo depth, and camera calibration information, all of which were obtained from \cite{endo-depth-and-motion}. Our methodology requires the use of tool masks to carry out spatiotemporal importance sampling. To this end, we employ a well-regarded vision foundation model known as Segment Anything. This model facilitates the semi-automatic segmentation of surgical instruments and the generation of corresponding masks.

% The Hamlyn dataset provides a rigorous test for our method as it incorporates sequences that image intracorporeal scenes. These scenes pose multiple challenges, including weak textures, deformations, reflections, surgical tool occlusions, and variations in illumination. Out of the entire Hamlyn dataset, we have specifically selected seven sequences, each of which contains 301 frames with a resolution of 480 $\times$ 640. Each of these sequences spans approximately 10 seconds and includes scenarios featuring surgical tool occlusion, extensive tissue mobilization, and large deformation, with some even displaying internal tissue exposure.
% We divide the frames of each sequence into two sets: a training set consisting of 151 frames, and an evaluation set comprising the remaining frames. This division allows us to adequately train our method while also providing a robust set for evaluation. 

\begin{figure}[tbp]
  \centering
  \begin{minipage}[t]{0.5\columnwidth}
    \centering
    \includegraphics[width=0.975\textwidth]{figures/endo}
    \label{fig:figure1}
  \end{minipage}%
  \begin{minipage}[t]{0.5\columnwidth}
    \centering
    \includegraphics[width=0.975\textwidth]{figures/ham}
    \label{fig:figure2}
  \end{minipage}
\caption{Visualization of datasets. The left column is from EndoNeRF dataset and the right is from Hamlyn dataset. From left to right is original image, tool mask and the binocular depth with tool mask.
% Visualization of the input data used in Forplane. The left column shows images from the EndoNeRF dataset, while the right column shows images from the Hamlyn dataset. The first image in each row represents the original image captured during surgery. The second image depicts the tool mask, highlighting the presence and location of surgical tools. The third image displays the masked ground-truth depth of the scene, providing depth information for the visible structures.
}
\label{fig: dataset}
\end{figure}

\begin{figure}[tbp]
\centerline{\includegraphics[width=1.0\columnwidth]{figures/performance_b2.pdf}}
\vspace{-0.5em}
\caption{Reconstruction results with difference maps. From left to right, we present the image rendered by Forplane, the corresponding ground truth image, and the difference map between them. These difference maps serve as a clear visual representation of our strong ability to reconstruct deformable tissues from tool-occluded endoscopy videos.
}
\vspace{-1.5em}
\label{fig: our performance b}
\end{figure}

% \subsection{Metrics}
% Given the impracticality of procuring a 3D tissue model or acquiring ground-truth depth with additional sensors in an in vivo environment due to clinical regulations, we resort to image-based metrics for the evaluation of our dynamic reconstruction results.
% Following~\cite{endonerf, edssr}, we use PSNR, SSIM and LPIPS for judging the performance of our dynamic reconstruction results. 
% To further enhance the comprehensiveness of our evaluation, we incorporate the FLIP metric~\cite{andersson2020flip,andersson2021visualizing}, which is used to measure the consistency of the underlying 3D scene. FLIP quantifies the number of pixels that alter in the image when viewed from the opposite side of the scene, thus offering a more inclusive evaluation of 3D reconstruction and rendering methodologies involving view synthesis.
% Note that the ground truth image contains occluded areas due to surgical tools, which may impact the overall evaluation metric. However, our main focus is on accurately reconstructing deformable tissues. To provide a clearer illustration of our method's effectiveness in tissue reconstruction, we introduce a modified metric called masked PSNR (PSNR*). This metric only measures the PSNR of tissue pixels rather than one image with masked area filling with zero, offering a more targeted assessment of our approach.

\begin{figure*}[htbp]
  \centering
%   \begin{minipage}[b]{0.18\textwidth}
%     \includegraphics[width=\linewidth]{figures/PSNR}
%     \label{fig:1}
%   \end{minipage}%
%   \hfill
  \begin{minipage}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figures/PSNR_star}
    \label{fig:5}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figures/SSIM}
    \label{fig:2}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figures/LPIPS}
    \label{fig:3}
  \end{minipage}%
  \hfill
  \begin{minipage}[b]{0.24\textwidth}
    \includegraphics[width=\linewidth]{figures/FLIPS}
    \label{fig:4}
  \end{minipage}%
  \caption{The Quantitative Comparison of Similarity Metrics for Reconstructed Volumes.
These figures present a quantitative comparison of similarity metrics between the input slices and the corresponding slices extracted from the reconstructed volumes. Four different similarity metrics, namely PSNR$^\star$, SSIM, LPIPS, FLIPS, are evaluated. Each figure depicts the performance of six different methods.}
  \label{fig:all}
% \vspace{-1.5em}
\end{figure*}

\begin{figure*}[htp]
% \vspace{-2em}
\centerline{\includegraphics[width=\textwidth]{LaTeX/figures/time_per_2line.pdf}}
% \vspace{-1em}
\caption{Results on the scene \textit{cutting twice} from EndoNeRF dataset~\cite{endonerf}. We present a comparison of tissue reconstructions from various methods. Forplane consistently shows more detailed reconstructions of the surgical procedure (\textit{e.g.} capillaries and peritoneum) compared to other methods.}
\label{fig: qualitative results}
% \vspace{-1.5em}
\end{figure*}

\subsection{Baselines}
We compare our approach with three state-of-the-art methods: EDSSR \cite{edssr}, EndoNeRF \cite{endonerf} and TiNeuVox \cite{tineuvox}. 
Each of these methods represents a different type of deformable tissue reconstruction. EDSSR \cite{edssr} leverages tissue deformation fields and volumetric fusion. EndoNeRF \cite{endonerf} utilizes dynamic neural radiance fields in MLPs to represent deformable surgical scenes and optimizes shapes and deformations in a learning-based manner. We follow the standard setting in~\cite{endonerf} with 200k optimizing iterations.
TiNeuVox \cite{tineuvox} integrates optimizable time-aware voxel features for faster optmization.
% tineuvox is not a medical structure!
Note that \cite{tineuvox} is not specified for surgical procedures, so we modify the original TiNeuVox model with tool mask-guided ray casting and stereo depth-cueing ray marching which are proposed by~\cite{endonerf}.
These methods are equipped with same hyper-parameters as~\cite{endonerf} and enables the TiNeuVox to reconstruct the dynamic tissues. We report two versions of TiNeuVox: TiNeuVox-S and TiNeuVox-B, representing the small and base versions, respectively. 
We also report Lerplane's performance~\cite{lerplane}, the previous version of Forplane. For fair comparison, we train Lerplane, TiNeuVox and Forplane with 32k iterations. 
We further report Forplane with only 9k iterations, showing significant optimization speed.

% \subsection{Implement Details}
% All experiments were conducted on an Ubuntu 20.04 system equipped with one NVIDIA GeForce RTX 3090 GPU. Forplane is implemented via pure pytorch~\cite{NEURIPS2019_9015}.
% To handle view-limited endoscopy videos, the scene was transformed into normalized device coordinates (NDC) for ray casting within this NDC space. The video duration was standardized to the range of $[-1, 1]$ based on frame numbers. Efficient ray marching employed occupancy grids with a resolution of 64, filtering out points with density below 1e-4 to reduce computational overhead.
% Spatiotemporal information was encoded using the Oneblob encoding method. The complete model consisted of four spatial resolution levels: 64, 128, 256, and 512 dimensions. Key hyperparameters included feature planes with $D=32$, spatiotemporal importance sampling with $j=25$, Oneblob encoding dimensionality of $\xi=16$, and the depth loss parameter of $\delta=0.05$. These hyperparameters were consistently applied across all experiments, unless otherwise specified. Optimization utilized the Adam optimizer with standard parameters. Each training iteration randomly sampled a batch of 2048 rays from the comprehensive dataset. The initial learning rate was set to 0.01, accompanied by a cosine schedule and a warming-up phase of 512 iterations. Training was performed for both 9k and 32k iterations, with training durations approximately lasting 3 and 10 minutes, respectively.

\subsection{Qualitative and Quantitative Results}
We show the quantitative results on EndoNeRF dataset in Fig.~\ref{fig:all} and all quantitative results on two datasets are summarized in Table~\ref{Tab: quantative} and Table~\ref{tab:time_speed}. All experiments were conducted on an Ubuntu 20.04 system equipped with one NVIDIA GeForce RTX 3090 GPU.
% claim
Four metrics are used for evaluation, $\textit{i.e.}$ PSNR, SSIM~\cite{ssim}, LPIPS~\cite{lpips}, FLIP~\cite{andersson2020flip}. These metrics are applied to the whole image including the masked empty areas. These areas may diminish the discernible differences between predicted and ground truth images. To address this, we introduce a modified metric called masked PSNR (PSNR*), which focuses solely on measuring the PSNR of tissue pixels, allowing for a more accurate comparison.
% Since the ground truth images contain occluded areas due to surgical tools, 
% To better compare the metrics on the reconstructed areas only, 
Apparently, Forplane outperforms other state-of-the-art methods across all evaluation metrics, demonstrating significantly superior performance. E-DSSR~\cite{edssr} achieves the fastest rendering speed due to its neural computing-light rendering procedure; however, its reconstruction quality is relatively low compared to other methods.
EndoNeRF~\cite{endonerf} shows promising reconstruction quality but requires approximately 14 hours for per-scene training. In contrast, our Forplane completes one scene learning in just 10 minutes while achieving better performance across all evaluation metrics. TiNeuVox-S~\cite{tineuvox} has a similar training time as Forplane-32k but exhibits significantly lower performance compared to our approach. TiNeuVox-B~\cite{tineuvox}, with a larger parameter quantity than TiNeuVox-S, exhibits stronger fitting ability. While better reconstruction quality is achieved on datasets with better quality (EndoNeRF dataset), the improvement diminishes on more challenging datasets (Hamlyn dataset). 
Furthermore, TiNeuVox-B accommodates a greater number of parameters, leading to increased computational time for both optimization and inference relative to TiNeuVox-S. In comparison, Forplane achieves high-quality reconstruction on both datasets with significantly faster rendering speed even with only 3 minutes optimization.
Our previous method~\cite{lerplane} exhibits performance akin to rapid optimization speeds, yet it lags in terms of rendering speed. Conversely, Forplane not only delivers superior overall quality but also boasts a rendering process that is roughly five times swifter than that of the previous version~\cite{lerplane}. This highlights the remarkable efficiency of our ray marching approach.
Furthermore, qualitative comparisons are provided in Fig.~\ref{fig: qualitative results} and the fine detailed reconstruction results are shown in Fig~\ref{fig: our performance a} and Fig.~\ref{fig: our performance b}.
The shared static field in Forplane enables better utilization of information throughout the surgical procedure, resulting in finer and more accurate details compared to other methods. Notably, Forplane achieves these improvements with less training time and faster rendering speed.

\begin{table*}[htp]
\centering
\caption{Mean values of quantitative metrics for different models on the two datasets (standard deviation in parentheses). \\$\uparrow$ indicates that higher values indicate higher accuracy, and vice versa.}
\label{Tab: quantative}
\begin{tabular}{l|ccccc}
\hline
Methods & PSNR$\uparrow$ & $\text{PSNR}^\star\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ \\
\hline
\multicolumn{6}{c}{EndoNeRF Dataset~\cite{endonerf}} \\
\hline
E-DSSR\cite{edssr} & 13.398 (1.270) & 12.997 (1.232) & 0.630 (0.057) & 0.423 (0.047) & 0.426 (0.056) \\
EndoNeRF\cite{endonerf} & 29.477 (1.886) & 28.560 (1.782) & 0.926 (0.021) & 0.080 (0.019) & 0.083 (0.014) \\
TiNeuVox-S\cite{tineuvox} & 29.913 (3.069) & 28.980 (2.862) & 0.919 (0.015) & 0.094 (0.015) & 0.083 (0.011) \\
TiNeuVox-B\cite{tineuvox} & 31.601 (2.855) & 30.668 (2.697) & \underline{0.940} (0.012) & \underline{0.064} (0.010) & \underline{0.067} (0.009) \\
Lerplane\cite{lerplane} & \underline{35.504} (1.161) & \underline{34.575} (1.129) & 0.935 (0.011) & 0.083 (0.009) & 0.075 (0.010) \\
Forplane-9k & 33.374 (1.074) & 32.435 (1.165) & 0.907 (0.014) & 0.127 (0.019) & 0.093 (0.007) \\
Forplane-32k & \textbf{37.306} (1.406) & \textbf{36.367} (1.521) & \textbf{0.945} (0.010) & \textbf{0.062} (0.008) & \textbf{0.063} (0.006) \\
\hline
\multicolumn{6}{c}{Hamlyn Dataset~\cite{hamlyn1, hamlyn2}} \\
\hline 
E-DSSR\cite{edssr} & 18.150 (2.571) & 17.337 (2.402) & 0.640 (0.060) & 0.393 (0.066) & 0.259 (0.065) \\
EndoNeRF\cite{endonerf} & 34.879 (1.784) & 34.066 (1.717) & 0.951 (0.011) & \underline{0.071} (0.017) & 0.070 (0.012) \\
TiNeuVox-S\cite{tineuvox} & 35.277 (1.682) & 34.464 (1.501) & \underline{0.953} (0.014) & 0.085 (0.029) & \underline{0.067} (0.016) \\
TiNeuVox-B\cite{tineuvox} & 33.764 (2.047) & 32.951 (1.974) & 0.942 (0.020) & 0.146 (0.061) & 0.078 (0.022) \\
Lerplane\cite{lerplane} & 32.455 (2.247) & 31.629 (2.064) & 0.935 (0.021) & 0.124 (0.041) & 0.098 (0.028) \\
Forplane-9k & \underline{35.301} (2.241) & \underline{34.475} (2.076) & 0.945 (0.018) & 0.093 (0.035) & 0.074 (0.020) \\
Forplane-32k & \textbf{37.474} (2.401) & \textbf{36.647} (2.232) & \textbf{0.960} (0.014) & \textbf{0.058} (0.025) & \textbf{0.059} (0.017) \\
\hline
\end{tabular}
% \vspace{-1.5em}
\end{table*}

\begin{table}[tbp]
\centering
\caption{Training Time and Test Speed for Different Methods}
\label{tab:time_speed}
\begin{tabular}{l|cc}
\hline
Methods & Train Time & Test Speed \\
\hline
E-DSSR\cite{edssr} & 13 mins & \textbf{28.0} fps \\
EndoNeRF\cite{endonerf} & $>$10 hours & 0.11 fps \\
TiNeuVox-S\cite{tineuvox} & 12 mins & 0.56 fps \\
TiNeuVox-B\cite{tineuvox} & 90 mins & 0.18 fps \\
Lerplane\cite{lerplane} & 10 mins & 0.38 fps \\
Forplane-9k & ~3 mins & \underline{1.73} fps \\
Forplane-32k & 10 mins & \underline{1.73} fps \\
\hline
\end{tabular}
\vspace{-1.5em}
\end{table}


Experimental results indicate that Forplane excels in computational speed and reconstruction quality, positioning it as a promising tool for future clinical and intraoperative applications in surgery. 
Through its pioneering method that bolsters optimization without sacrificing the quality of reconstruction, Forplane stands poised to transform the landscape of surgical procedures.

\subsection{Ablation Study}
In this section, we perform a series of experiments to validate the effectiveness of our proposed methods. The experiments are conducted on the EndoNeRF dataset~\cite{endonerf} with 9k iterations, and the reported metric values are averaged.

\noindent \textbf{Sampling Strategy}
% \subsubsection{Sampling Strategy}
We compare our proposed spatiotemporal importance sampling strategy with two other sampling strategies: Naive Sampling, which avoids tool masks and assigns equal weights to all pixels, and EndoNeRF Sampling, which assigns higher probabilities to highly occluded areas as described in \cite{endonerf}.

\noindent \textbf{Encoding Method}
% \subsubsection{Encoding}
We compare our coordinate-time encoding method with two methods: Dummy Encoding, which replaces all the coordinate-time encoded parameters with a constant value to preserve the parameter quantity of the tiny MLP, and Direction Encoding, where one-blob positional encoding is applied to the view direction and the encoded parameters are passed to the tiny MLP, as described in \cite{nerf}.

\noindent \textbf{Space-time Disentangle}
% \subsubsection{Space-time Disentangle}
As detailed in Sec.~\ref{Disentangle Loss}, we use a specialized initialization for $\mathbf{V}_{3d}^d$ and pair it with $\mathcal{L}_{DE}$ to enhance the decomposition between $\mathbf{V}_{3d}^d$ and $\mathbf{V}_{3d}^s$. For comparison, we also trained a version of Forplane without these adjustments, termed w/o Disentangle.

\noindent \textbf{Ray Marching}
% In this improved version, we introduce one efficient ray marching algorithm to generate accurate spatial-temporal points for interpolation. To ablate this ray marching algorithm, we provide a comparative evaluation against two alternative methods: the sample-net method (termed Sample-Net) and the stereo depth-cueing ray marching method (termed Depth-Cueing). The sample-net method is proposed by the original version~\cite{lerplane}, which employs a simplified 4D scene representation to provides more accurate sampling.
% The stereo depth-cueing ray marching method is proposed in EndoNeRF~\cite{endonerf}, which create Gaussian transfer functions with stereo depth to guide point sampling near tissue surfaces.
In this improved version, we introduce an efficient ray marching algorithm designed to accurately generate spatial-temporal points. To evaluate the effectiveness of this algorithm, we conducted a comparative analysis against two existing methods: the sample-net method (termed Sample-Net) and the stereo depth-cueing ray marching method (termed Depth-Cueing). Sample-Net, as proposed in the original version of our work~\cite{lerplane}, utilizes a simplified representation of the 4D scene, aiming to enhance the accuracy of point sampling. In contrast, the Depth-Cueing method, introduced in EndoNeRF~\cite{endonerf}, employs Gaussian transfer functions informed by stereo depth data to guide the sampling of points near tissue surfaces, aiming to optimize the rendering of fine details.

\begin{table}[tbp]
\centering
\caption{Mean values of evaluation metrics for different ablation models on the EndoNeRF~\cite{endonerf} dataset.}
\label{tab: ablation}
\begin{tabular}{l|ccccc}
\hline
Methods & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ \\
\hline
Naive Sampling  & 33.146 & 0.906 & 0.135 & 0.094 \\
EndoNeRF Sampling  & 33.019 & 0.906 & 0.135 & 0.093 \\
Dummy Encoding  & 33.055 & 0.905 & 0.129 & 0.094 \\
Direction Encoding  & 33.062 & 0.904 & 0.133 & 0.095 \\
W/o Disentangle & 18.015 & 0.869 & 0.302 & 0.349 \\
\hline
Full Model  & 33.374 & 0.907 & 0.127 & 0.093 \\
\hline
\end{tabular}
% \vspace{-1.5em}
\end{table}

\begin{figure*}[tbp]
\centerline{\includegraphics[width=\textwidth]{LaTeX/figures/lambda_new.pdf}}
\caption{Comparative reconstruction results with varied weighting parameters. This figure illustrates the performance impact of different weighting configurations on the reconstruction process, with the horizontal axis represented in a logarithmic scale. Fig.~9 (a) shows the performance of Forplane with different $\lambda_d$. Fig.~9 (b) shows $\lambda_{tv}$, Figure (c) shows $\lambda_{ts}$ and Figure (d) shows $\lambda_{de}$.
}
\label{fig: lambda}
\end{figure*}

\begin{table}[tbp]
\centering
\caption{Evaluation metrics for different ray marching strategy on the EndoNeRF~\cite{endonerf} dataset.}
\label{tab: ablation ray marching}
\begin{tabular}{l|ccccc}
\hline
Methods & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Test Speed$\uparrow$ \\
\hline
Depth-Cueing &	31.325 &	0.897 &	0.132 & 1.95 fps \\
Sample-Net	&32.889	&0.901	&0.126	&0.38 fps \\
Ours	&33.374&	0.907&	0.127&	1.73 fps \\
\hline
\end{tabular}
\end{table}

The results of the ablation study are summarized in Table~\ref{tab: ablation} and Table~\ref{tab: ablation ray marching}. Our spatiotemporal importance sampling achieves superior quality compared to the other sampling strategies, confirming its effectiveness. Regarding encoding methods, our coordinate-time encoding outperforms the others, while the performance of Dummy and Direction Encoding is similar, validating of our hypothesis in Section \ref{method: Coordinate-Time Encoding}.
Forplane w/o Disentangle shows notable degradation, primarily from optimization ambiguities. Lacking clear guidance on decomposition, the network struggles to distinguish between static and dynamic elements given the restricted viewpoints.
The results presented in Table~\ref{tab: ablation ray marching} indicate that the depth-cueing method yields suboptimal performance, primarily due to the reliance on noisy and incomplete stereo depth data, as depicted in Fig.~\ref{fig: dataset}. Additionally, its inapplicability for temporal interpolation further limits its utility due to the absence of stereo depth in certain contexts. Conversely, while the sample-net method is versatile, it leads to increased computational demands during inference, negatively impacting test speed.
Our efficient ray marching method effectively mitigates these issues, striking a balance between rendering speed and reconstruction quality. It outperforms the depth-cueing method in terms of PSNR and SSIM, and also surpasses the sample-net method in inference speed, thus demonstrating its potential for real-time application scenarios.

\begin{table}[tbp]
\centering
\caption{The performance between Forplane and MForplane. The time row represents for optimization time.}
\label{tab: monocular}
\begin{tabular}{l|ccccc}
\hline
Methods & PSNR$\uparrow$ & $\text{PSNR}^\star\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ \\
\hline
\multicolumn{6}{c}{EndoNeRF Dataset~\cite{endonerf}} \\
\hline
Forplane & 37.306 & 36.367 & 0.945 & 0.062 & 0.063 \\
MForplane  & 36.403 & 35.464 & 0.938 & 0.073 & 0.071 \\
\hline
\multicolumn{6}{c}{Hamlyn Dataset~\cite{hamlyn1, hamlyn2}} \\
\hline
Forplane & 37.474 & 36.647  & 0.960  & 0.058  & 0.059  \\
MForplane  & 37.034 & 36.208 & 0.959 & 0.060 & 0.063 \\
\hline
\end{tabular}
\end{table}

\subsection{Hyperparameters}
As delineated in Section~\ref{method: Optimization}, we set the $\lambda$ parameters to a specific weighting configuration across all experiments. This subsection is dedicated to conducting a comprehensive analysis to discern the effects of various hyperparameters on Forplane's performance. To this end, we train Forplane using an array of $\lambda$ weightings on the EndoNeRF dataset~\cite{endonerf}, extending across 32k iterations. The results, depicted in Fig.~\ref{fig: lambda}, suggest that Forplane exhibits considerable robustness to variations in loss weighting configurations, only excessively large weightings could potentially impair performance.


\subsection{Monocular Reconstruction}
We show the performance of MForplane and Forplane on two datasets in Table.~\ref{tab: monocular}. By incorporating depth priors from monocular depth estimation networks, MForplane achieves fast reconstruction of dynamic tissues in monocular endoscopic videos. However, when compared to Forplane, we observe a slight decrease in the reconstruction quality of MForplane (\textit{e.g.} 1.81\% in PSNR, 0.4\% in SSIM).
Furthermore, there is a slight increase in the training time (from 10 minutes to 12 minutes), primarily attributed to the additional computational workload involved in calculating the monocular depth loss. Nevertheless, it is important to note that the ability to achieve fast reconstruction of dynamic tissues using one monocular endoscopic video holds significant promise for various applications in medical imaging. Therefore, the minor reduction in quality is deemed acceptable given the enormous potential and practicality of MForplane.


\subsection{The Choice of MLP Structure}
% In Section \ref{method: Neural Forplane Representation for Deformable Tissues}, we introduce a fast orthogonal plane representation that reduces the computational load on the Multilayer Perceptron (MLP), allowing for a more efficient MLP architecture in complex surgical reconstruction tasks. To validate this approach, we conducted an experimental comparison where our model's MLP was replaced with the more elaborate MLP structure utilized by EndoNeRF~\cite{endonerf}. The experimental results, detailed in Table~\ref{tab: ablation MLP}, indicate that the use of a larger MLP configuration does not significantly enhance reconstruction quality but results in a substantial increase in training duration for the same iteration count. These outcomes strongly corroborate our proposition that a streamlined MLP architecture contributes to enhanced optimization and inference efficiency, underscoring the effectiveness of our proposed method."
As mentioned in Section \ref{method: Neural Forplane Representation for Deformable Tissues}, our fast orthogonal plane representation reduces the computational load on the MLP, allowing for a more efficient MLP architecture in complex surgical reconstruction tasks. To validate this approach, we conducted an experimental comparison where our tiny MLP (2 fully-connected ReLU layers with 64 channels) was replaced with the more elaborate MLP structure (8 fully-connected ReLU layers with 256 channels) utilized by EndoNeRF~\cite{endonerf}. The experiments are conducted on the EndoNeRF dataset with 9k iterations, and the reported metric values are averaged. The experimental results, detailed in Table~\ref{tab: ablation MLP}, indicate that the use of a larger MLP configuration does not significantly enhance reconstruction quality but results in a substantial increase in training duration for the same iteration count. These outcomes strongly corroborate our proposition that a streamlined MLP architecture contributes to enhanced optimization and inference efficiency, underscoring the effectiveness of our proposed method.

\begin{table}[tbp]
\centering
\caption{Mean values of evaluation metrics for different MLP structure on the EndoNeRF~\cite{endonerf} dataset.}
\label{tab: ablation MLP}
\begin{tabular}{l|cccc}
\hline
Methods & PSNR$\uparrow$ & SSIM$\uparrow$ & Train Time$\downarrow$ & Test Speed$\uparrow$ \\
\hline
Large MLP  & 34.285 & 0.913 & 23 mins & 0.75 fps \\
Tiny MLP  & 33.374 & 0.907 & ~3 mins & 1.73 fps \\
\hline
\end{tabular}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.975\columnwidth]{LaTeX/figures/spacetime_edit_v2}}
\caption{Visualization of static and dynamic fields. 
The visualizations provided demonstrate the decomposition of static and dynamic fields in surgical procedures, showcasing the effectiveness of utilizing scene context within Forplane. The first image of each row shows the result of full 4D volume. The second image corresponds to the static field, while the third image portrays the dynamic field, which is re-normalized to [0, 1] for optimal visualization.}
\label{fig: decomposition}
\end{figure}

\subsection{Disentangle Static and Dynamic Field}
We propose an effective method for visualizing the static and dynamic fields in surgical scenes, showcasing the efficacy of our factorization approach.
Our approach utilizes element-wise multiplication for feature aggregation across different feature planes, as outlined in Eq.~\ref{eq:interpolate}. 
By setting all values in the dynamic field to 1 and performing inference, we obtain the network's output as the rendered result of the static field. Similarly, setting all values in the static field to 1 provides the rendered result of the dynamic field. 
% Fig.~\ref{fig: decomposition} shows the visualization of static field and dynamic field decomposition. 
The time-space decomposition is clearly illustrated in Fig.~\ref{fig: decomposition}, offering a compelling demonstration of the effectiveness of our proposed structure. 
This property offers valuable insights into tissue examination and procedural understanding during surgery, with potential applications in virtual surgery and intraoperative utilization.

% The ability to delineate static elements from dynamic movements during surgical procedures provides surgeons with a powerful tool to augment tissue examination, enrich procedural understanding, and mitigate the risk of unnoticed pathologies or accidental harm to normal structures. This implicit articulation of static and dynamic components forms a strong underpinning for applications such as virtual surgery, showcasing considerable potential for intraoperative utilization.


% We propose a natural and effective method for visualizing the static and dynamic fields, showcasing the efficacy of our factorization approach. In section~\ref{method: Neural Forplane Representation for Deformable Tissues} and Eq.~\ref{eq: disentangle loss}, we describe the process of segregating the static field from the surgical scenes using a simple yet powerful disentanglement regularization. However, the immediate impact of this disentanglement is not easily observable. To address this challenge, we introduce an insightful algorithm that enables the visualization of our static-dynamic separation, which has remained elusive to existing methods.

% Our approach utilizes element-wise multiplication for feature aggregation across different feature planes, as outlined in Eq.~\ref{eq:interpolate}. By setting all values in the dynamic field to 1 and performing inference, we obtain the network's output as the rendered result of the static field. Similarly, setting all values in the static field to 1 provides the rendered result of the dynamic field. This time-space decomposition is clearly illustrated in Fig.~\ref{fig: decomposition}, offering a compelling demonstration of the effectiveness of our proposed structure.

% The ability to delineate static elements from dynamic movements during surgical procedures provides surgeons with a powerful tool to augment tissue examination, enrich procedural understanding, and mitigate the risk of unnoticed pathologies or accidental harm to normal structures. This implicit articulation of static and dynamic components forms a strong underpinning for applications such as virtual surgery, showcasing considerable potential for intraoperative utilization.

% Our static-dynamic field structure naturally disentangles dynamic and static portions of the scene. 

% enables high quality deformable tissues reconstruction 


% \begin{figure}[!t]
% \centerline{\includegraphics[width=\columnwidth]{fig1.png}}
% \caption{Magnetization as a function of applied field.
% It is good practice to explain the significance of the figure in the caption.}
% \label{fig: demo}
% \end{figure}



==> LaTeX/4_results.tex <==
\section{Guidelines for Graphics Preparation and Submission}
\label{sec:guidelines}

\subsection{Types of Graphics}
The following list outlines the different types of graphics published in 
IEEE journals. They are categorized based on their construction, and use of 
color~/~shades of gray:

\subsubsection{Color/Grayscale figures}
{Figures meant to appear in color, or shades of black/gray. Such 
figures may include photographs, illustrations, multicolor graphs, and 
flowcharts.}

\subsubsection{Line Art figures}
{Figures that are composed of only black lines and shapes. These figures 
should have no shades or half-tones of gray, only black and white.}

\subsubsection{Author photos}
{Not allowed for papers in TMI.}

\subsubsection{Tables}
{Data charts which are typically black and white, but sometimes include 
color.}

\begin{table}
\caption{Units for Magnetic Properties}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
\hline
Symbol& 
Quantity& 
Conversion from Gaussian and \par CGS EMU to SI $^{\mathrm{a}}$ \\
\hline
$\Phi $& 
magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V$\cdot $s \\
$B$& 
magnetic flux density, \par magnetic induction& 
1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
$H$& 
magnetic field strength& 
1 Oe $\to  10^{3}/(4\pi )$ A/m \\
$m$& 
magnetic moment& 
1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A$\cdot $m$^{2} = 10^{-3}$ J/T \\
$M$& 
magnetization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{3}$ A/m \\
4$\pi M$& 
magnetization& 
1 G $\to  10^{3}/(4\pi )$ A/m \\
$\sigma $& 
specific magnetization& 
1 erg/(G$\cdot $g) $=$ 1 emu/g $\to $ 1 A$\cdot $m$^{2}$/kg \\
$j$& 
magnetic dipole \par moment& 
1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb$\cdot $m \\
$J$& 
magnetic polarization& 
1 erg/(G$\cdot $cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
$\chi , \kappa $& 
susceptibility& 
1 $\to  4\pi $ \\
$\chi_{\rho }$& 
mass susceptibility& 
1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
$\mu $& 
permeability& 
1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A$\cdot $m) \\
$\mu_{r}$& 
relative permeability& 
$\mu \to \mu_{r}$ \\
$w, W$& 
energy density& 
1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
$N, D$& 
demagnetizing factor& 
1 $\to  1/(4\pi )$ \\
\hline
\multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
the entire table do not need footnote letters. }\\
\multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
$=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
kilogram, H $=$ henry.}
\end{tabular}
\label{tab1}
\end{table}

\subsection{Multipart figures}
Multipart figures are comprised of more than one sub-figure presented together.
If a multipart figure is made up of multiple figure types (one part is lineart,
and another is grayscale or color) the figure should meet the strictest applicable guidelines.

\subsection{File Formats For Graphics}
\label{formats}
Format and save your graphics as one of the following approved file types:
PostScript (.PS), Encapsulated PostScript (.EPS), Tagged Image File Format (.TIFF),
Portable Document Format (.PDF), Portable Network Graphics (.PNG), or Metapost (.MPS).
After the paper is accepted, any included graphics must be submitted alongside the final manuscript files.

\subsection{Sizing of Graphics}
Most charts, graphs, and tables are one column wide (3.5 inches~/~88 
millimeters) or page wide (7.16 inches~/~181 millimeters). The maximum
depth of a graphic is 8.5 inches (216 millimeters). When choosing the depth of a graphic,
please allow space for a caption. Authors are allowed to size figures between column and
page widths, but it is recommended not to size figures less than column width unless necessary. 

\subsection{Resolution}
The proper resolution of your figures will depend on the type of figure it 
is as defined in the ``Types of Figures'' section. Author photographs, 
color, and grayscale figures should be at least 300dpi. Lineart, including 
tables should be a minimum of 600dpi.

\subsection{Vector Art}
While IEEE does accept and even recommends that authors submit artwork
in vector format, it is our policy is to rasterize all figures for publication. This is done
in order to preserve figures' integrity across multiple computer platforms.

\subsection{Colorspace}
The term colorspace refers to the entire sum of colors that can be 
represented within a given medium. For our purposes, the three main colorspaces
are grayscale, RGB (red/green/blue) and CMYK (cyan/magenta/yellow/black).
RGB is generally used with on-screen graphics, whereas CMYK is used for printing purposes.

All color figures should be generated in RGB or CMYK colorspace. Grayscale 
images should be submitted in grayscale colorspace. Line art may be 
provided in grayscale OR bitmap colorspace. Note that ``bitmap colorspace'' 
and ``bitmap file format'' are not the same thing. When bitmap colorspace 
is selected, .TIF/.TIFF are the recommended file formats.

\subsection{Accepted Fonts Within Figures}
When preparing your graphics IEEE suggests that you use of one of the 
following Open Type fonts: Times New Roman, Helvetica, Arial, Cambria, and 
Symbol. If you are supplying EPS, PS, or PDF files all fonts must be 
embedded. Some fonts may only be native to your operating system; without 
the fonts embedded, parts of the graphic may be distorted or missing.

A safe option when finalizing your figures is to strip out the fonts before 
you save the files, creating ``outline'' type. This converts fonts to 
artwork that will appear uniformly on any screen.

\subsection{Using Labels Within Figures}

\subsubsection{Figure Axis labels}
Figure axis labels are often a source of confusion. Use words rather than 
symbols. As an example, write the quantity ``Magnetization,'' or 
``Magnetization M,'' not just ``M.'' Put units in parentheses. Do not label 
axes only with units. As in Fig. 1, for example, write ``Magnetization 
(A/m)'' or ``Magnetization (A$\cdot$m$^{-1}$),'' not just ``A/m.''
Do not label axes with a ratio of quantities and units.
For example, write ``Temperature (K),'' not ``Temperature/K.'' 

Multipliers can be especially confusing. Write ``Magnetization (kA/m)'' or 
``Magnetization (10$^{3}$ A/m).'' Do not write ``Magnetization 
(A/m)$\,\times\,$1000'' because the reader would not know whether the top 
axis label in Fig. 1 meant 16000 A/m or 0.016 A/m. Figure labels should be 
legible, approximately 8 to 10 point type.

\subsubsection{Subfigure Labels in Multipart Figures and Tables}
Multipart figures should be combined and labeled before final submission. 
Labels should appear centered below each subfigure in 8 point Times New 
Roman font in the format of (a) (b) (c).

\subsection{Referencing a Figure or Table Within Your Paper}
When referencing your figures and tables within your paper, use the 
abbreviation ``Fig.'' even at the beginning of a sentence. Do not abbreviate 
``Table.'' Tables should be numbered with Roman numerals.

\subsection{Submitting Your Graphics}
Format your paper with the graphics included within the body of the text
as you would expect to see the paper in print. Please do this at each stage of the review,
from first submission to final files. For final files only, after the paper has been accepted
for publication, figures should also be submitted individually in addition to the manuscript
file using one of the approved file formats. Place a figure caption below each figure;
place table titles above the tables. Do not include captions or borders in the uploaded figure files.

\subsection{File Naming}
Figures (line artwork or images) should be named starting with the 
first 5 letters of the corresponding author's last name. The next characters in the 
filename should be the number that represents the figure's sequential 
location in the article. For example, in author ``Anderson's'' paper,
the first three figures might be named ander1.tif, ander2.tif, and ander3.ps.

Tables should contain only the body of the table (not the caption) and 
should be named similarly to figures, except that `.t' is inserted 
in-between the author's name and the table number. For example, author 
Anderson's first three tables would be named ander.t1.tif, ander.t2.ps, ander.t3.eps.

Author photographs or biographies are not permitted in IEEE TMI papers.

\subsection{Checking Your Figures: The IEEE Graphics Analyzer}
The IEEE Graphics Analyzer enables authors to pre-screen their graphics for 
compliance with IEEE Transactions and Journals standards before submission. 
The online tool, located at \underline{http://graphicsqc.ieee.org/},
allows authors to upload their graphics in order to check that each file is the correct file format,
resolution, size and colorspace; that no fonts are missing or corrupt;
that figures are not compiled in layers or have transparency,
and that they are named according to the IEEE Transactions and Journals naming convention.
At the end of this automated process, authors are provided with 
a detailed report on each graphic within the web applet, as well as by email.

For more information on using the Graphics Analyzer or any other graphics 
related topic, contact the IEEE Graphics Help Desk by e-mail at 
graphics@ieee.org.

\subsection{Color Processing/Printing in IEEE Journals}
All IEEE Transactions, Journals, and Letters allow an author to publish 
color figures on IEEE Xplore\textregistered\ at no charge, and automatically 
convert them to grayscale for print versions. In most journals, figures and 
tables may alternatively be printed in color if an author chooses to do so. 
Please note that this service comes at an extra expense to the author. If 
you intend to have print color graphics, include a note with your final 
paper indicating which figures or tables you would like to be handled that way,
and stating that you are willing to pay the additional fee.

\section{Some Common Mistakes}
The word ``data'' is plural, not singular. The subscript for the 
permeability of vacuum $\mu _{0}$ is zero, not a lowercase letter 
``o.'' Use the word ``micrometer'' instead of ``micron.'' A graph within a graph is an 
``inset,'' not an ``insert.'' The word ``alternatively'' is preferred to the 
word ``alternately'' (unless you really mean something that alternates). Use 
the word ``whereas'' instead of ``while'' (unless you are referring to 
simultaneous events). Do not use the word ``essentially'' to mean 
``approximately'' or ``effectively.'' Do not use the word ``issue'' as a 
euphemism for ``problem.'' When compositions are not specified, separate 
chemical symbols by en-dashes; for example, ``NiMn'' indicates the 
intermetallic compound Ni$_{0.5}$Mn$_{0.5}$ whereas 
``Ni--Mn'' indicates an alloy of some composition 
Ni$_{x}$Mn$_{1-x}$.

Be aware of the different meanings of the homophones ``affect'' (usually a 
verb) and ``effect'' (usually a noun), ``complement'' and ``compliment,'' 
``discreet'' and ``discrete,'' ``principal'' (e.g., ``principal 
investigator'') and ``principle'' (e.g., ``principle of measurement''). Do 
not confuse ``imply'' and ``infer.'' 

Prefixes such as ``non,'' ``sub,'' ``micro,'' ``multi,'' and ``ultra'' are 
not independent words; they should be joined to the words they modify, 
usually without a hyphen. There is no period after the ``et'' in the Latin 
abbreviation ``\emph{et al.}'' (it is also italicized). The abbreviation ``i.e.,'' means 
``that is,'' and the abbreviation ``e.g.,'' means ``for example'' (these 
abbreviations are not italicized).

A general IEEE styleguide is available at \underline{http://www.ieee.org/web/publications/authors/transjnl/index.ht}
\discretionary{}{}{}\underline{ml}.

==> LaTeX/5_discussion.tex <==
\section{Discussion}
Forplane exhibits SOTA performance in rapidly reconstructing high-quality deformable tissues within both monocular and binocular endoscopic videos. This significant advancement is attributed to a series of critical observations and methodological innovations:
1) Combination of Implicit and Explicit Representations: While implicit representations excel in detailed scene restoration, the computational demands are substantial. Conversely, explicit representations, though computationally efficient, often lack detail. Forplane integrates the strengths of both implicit and explicit representations, thereby achieving efficient training and inference, alongside high-quality reconstruction.
2) Selective Focus on Significant Regions: Acknowledging the varying significance of different tissues, Forplane strategically focuses on critical regions. This targeted approach accelerates the optimization process by allocating computational resources to areas of the scene with the most impact on overall reconstruction quality.
3) Utilization of Temporal Information: Given the limited viewpoint in endoscopic environments, Forplane effectively leverages temporal data. This utilization of temporal information is key in enhancing the accuracy of the reconstruction, particularly in dynamically changing surgical scenes.
% 3) Hybrid Representation Approach. By integrating explicit representations with implicit models, Forplane not only boosts reconstruction quality but also markedly accelerates optimization.

Despite its notable achievements, Forplane has areas that warrant further development. First, the MForplane variant, designed to operate without stereo depth, still depends on manually generated masks for surgical instrument identification. This process is both challenging and labor-intensive, highlighting the need for advancements in automated instrument labeling and tracking.
Secondly, the rendering speed of Forplane, although significantly faster than its predecessor (approximately 5 times quicker at 1.73 fps on a single RTX3090 GPU), does not yet meet the demands for real-time intraoperative assistance. This limitation underscores the necessity for further improvements in rendering speed.
Lastly, the functionality of Forplane is presently focused on the reconstruction of deformable tissues. To fully support comprehensive surgical training for robotic systems, a more detailed analysis of surgical procedures is required. This includes not only deformable tissue reconstruction but also the intricate dynamics of surgical instruments, environmental lighting conditions, and camera motion.

\section{Conclusion}
In this paper, we propose a fast dynamic reconstruction framework, Forplane, targeted on deformable tissues during surgery. 
% With a monocular optimizing strategy, our MForplane shows remarkable reconstruction performance on monocular endoscopy videos.
% \repd{
Forplane represents surgical procedures with orthogonal neural planes and incorporates advancements in pixel sampling, spatial sampling, and information enhancement to improve rendering quality, accelerate optimization and inference. 
Evaluations on two in vivo datasets demonstrate the superior performance of Forplane, requiring less training time and offering faster inference speed compared to other methods.
In addition, Forplane effectively handles both monocular and binocular endoscopy videos, maintaining nearly identical high-quality reconstruction performance.
% }{
% Compared to previous methods, Forplane has the following significant contributions:
% \begin{itemize}
% \item Orthogonal Neural Plane Representation: It models surgical procedures using orthogonal neural planes, enhancing the precision and effectiveness of the reconstruction.
% \item Advancements in Sampling and Information Enhancement: Incorporates cutting-edge techniques in pixel sampling, spatial sampling, and information enhancement to significantly improve rendering quality, accelerate optimization and speed up inference. 
% % \item Accelerated Optimization and Inference: Forplane streamlines the optimization process and speeds up inference, leading to more efficient performance.
% \item Superior Performance Validated by In Vivo Studies: Demonstrates better performance than other methods in terms of training time and inference speed, as validated by evaluations on two in vivo datasets.
% % \item Versatility in Video Analysis: Capable of effectively handling both monocular and binocular endoscopy videos without compromising on the quality of reconstruction.
% \item High-Quality Reconstruction: Maintains nearly identical, high-quality reconstruction performance, making it highly reliable.
% \end{itemize}
% }
We firmly believe that Forplane holds substantial promise for intraoperative applications among surgery.

==> LaTeX/6_acknowledge.tex <==
% \appendices

% \section*{Appendix and the Use of Supplemental Files}
% Appendices, if needed, appear before the acknowledgment. If an appendix is not
% critical to the main message of the manuscript and is included only for thoroughness
% or for reader reference, then consider submitting appendices as supplemental materials.
% Supplementary files are available to readers through IEEE \emph{Xplore\textregistered}
% at no additional cost to the authors but they do not appear in print versions.
% Supplementary files must be uploaded in ScholarOne as supporting documents, but for
% accepted papers they should be uploaded as Multimedia documents. Refer readers
% to the supplementary files where appropriate within the manuscript text using footnotes.
% \footnote{Supplementary materials are available in the supporting documents/multimedia tab.
% Further instructions on footnote usage are in the Footnotes section on the next page.}

% \section*{Acknowledgment}
% The preferred spelling of the word ``acknowledgment'' in American English is 
% without an ``e'' after the ``g.'' Use the singular heading even if you have 
% many acknowledgments. Avoid expressions such as ``One of us (S.B.A.) would 
% like to thank $\ldots$ .'' Instead, write ``F. A. Author thanks $\ldots$ .'' In most 
% cases, sponsor and financial support acknowledgments are placed in the 
% unnumbered footnote on the first page, not here.

==> LaTeX/egbib_all.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@article{nerf,
  title={Nerf: Representing scenes as neural radiance fields for view synthesis},
  author={Mildenhall, Ben and Srinivasan, Pratul P and Tancik, Matthew and Barron, Jonathan T and Ramamoorthi, Ravi and Ng, Ren},
  journal={Communications of the ACM},
  year={2021},
}

@inproceedings{endonerf,
  title={Neural rendering for stereo 3d reconstruction of deformable tissues in robotic surgery},
  author={Wang, Yuehao and Long, Yonghao and Fan, Siu Hin and Dou, Qi},
  booktitle={MICCAI},
  year={2022},
}

@article{endo-depth-and-motion,
  title={Endo-depth-and-motion: reconstruction and tracking in endoscopic videos using depth networks and photometric constraints},
  author={Recasens, David and Lamarca, Jos{\'e} and F{\'a}cil, Jos{\'e} M and Montiel, JMM and Civera, Javier},
  journal={RA-L},
  year={2021},
}

@inproceedings{edssr,
  title={E-dssr: efficient dynamic surgical scene reconstruction with transformer-based stereoscopic depth perception},
  author={Long, Yonghao and Li, Zhaoshuo and Yee, Chi Hang and Ng, Chi Fai and Taylor, Russell H and Unberath, Mathias and Dou, Qi},
  booktitle={MICCAI},
  year={2021},
}

@article{andersson2020flip,
  title={FLIP: A Difference Evaluator for Alternating Images.},
  author={Andersson, Pontus and Nilsson, Jim and Akenine-M{\"o}ller, Tomas and Oskarsson, Magnus and {\AA}str{\"o}m, Kalle and Fairchild, Mark D},
  journal={PACMCGIT},
  year={2020}
}

@article{andersson2021visualizing,
  title={Visualizing errors in rendered high dynamic range images},
  author={Andersson, Pontus and Nilsson, Jim and Shirley, Peter and Akenine-M{\"o}ller, Tomas},
  year={2021},
  journal={Eurographics},
}

@article{stasis,
  title={StaSiS-Net: A stacked and siamese disparity estimation network for depth reconstruction in modern 3D laparoscopy},
  author={Bardozzo, Francesco and Collins, Toby and Forgione, Antonello and Hostettler, Alexandre and Tagliaferri, Roberto},
  journal={MIA},
  year={2022},
}

@article{lerplane,
  title={Neural LerPlane Representations for Fast 4D Reconstruction of Deformable Tissues},
  author={Yang, Chen and Wang, Kailing and Wang, Yuehao and Yang, Xiaokang and Shen, Wei},
  journal={MICCAI},
  year={2023}
}

@article{song2017dynamic,
  title={Dynamic reconstruction of deformable soft-tissue with stereo scope in minimal invasive surgery},
  author={Song, Jingwei and Wang, Jun and Zhao, Liang and Huang, Shoudong and Dissanayake, Gamini},
  journal={RA-L},
  year={2017},
}

@article{zhou2019real,
  title={Real-time dense reconstruction of tissue surface from stereo optical video},
  author={Zhou, Haoyin and Jagadeesan, Jayender},
  journal={TMI},
  year={2019},
}

@inproceedings{zhou2021emdq,
  title={EMDQ-SLAM: Real-time high-resolution reconstruction of soft tissue surface from stereo laparoscopy videos},
  author={Zhou, Haoyin and Jayender, Jagadeesan},
  booktitle={MICCAI},
  year={2021},
}

@article{li2020super,
  title={Super: A surgical perception framework for endoscopic tissue manipulation with surgical robotics},
  author={Li, Yang and Richter, Florian and Lu, Jingpei and Funk, Emily K and Orosco, Ryan K and Zhu, Jianke and Yip, Michael C},
  journal={RA-L},
  year={2020},
}

@inproceedings{li20213d,
  title={3D Ultrasound Spine Imaging with Application of Neural Radiance Field Method},
  author={Li, Honggen and Chen, Hongbo and Jing, Wenke and Li, Yuwei and Zheng, Rui},
  booktitle={IUS},
  year={2021},
}

@inproceedings{khan2022implicit,
  title={Implicit Neural Representations for Medical Imaging Segmentation},
  author={Khan, Muhammad Osama and Fang, Yi},
  booktitle={MICCAI},
  year={2022},
}

@inproceedings{yang2022implicitatlas,
  title={ImplicitAtlas: learning deformable shape templates in medical imaging},
  author={Yang, Jiancheng and Wickramasinghe, Udaranga and Ni, Bingbing and Fua, Pascal},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{corona2022mednerf,
  title={Mednerf: Medical neural radiance fields for reconstructing 3d-aware ct-projections from a single x-ray},
  author={Corona-Figueroa, Abril and Frawley, Jonathan and Bond-Taylor, Sam and Bethapudi, Sarath and Shum, Hubert PH and Willcocks, Chris G},
  booktitle={EMBC},
  year={2022},
}

@article{schwarz2020graf,
  title={Graf: Generative radiance fields for 3d-aware image synthesis},
  author={Schwarz, Katja and Liao, Yiyi and Niemeyer, Michael and Geiger, Andreas},
  journal={NeurIPS},
  year={2020}
}

@article{ruckert2022neat,
  title={Neat: Neural adaptive tomography},
  author={R{\"u}ckert, Darius and Wang, Yuanhao and Li, Rui and Idoughi, Ramzi and Heidrich, Wolfgang},
  journal={TOG},
  year={2022},
}

@inproceedings{fang2022curvature,
  title={Curvature-Enhanced Implicit Function Network for High-quality Tooth Model Generation from CBCT Images},
  author={Fang, Yu and Cui, Zhiming and Ma, Lei and Mei, Lanzhuju and Zhang, Bojun and Zhao, Yue and Jiang, Zhihao and Zhan, Yiqiang and Pan, Yongsheng and Zhu, Min and others},
  booktitle={MICCAI},
  year={2022},
}

@inproceedings{raju2022deep,
  title={Deep implicit statistical shape models for 3d medical image delineation},
  author={Raju, Ashwin and Miao, Shun and Jin, Dakai and Lu, Le and Huang, Junzhou and Harrison, Adam P},
  booktitle={AAAI},
  year={2022}
}

@article{sun2021coil,
  title={Coil: Coordinate-based internal learning for tomographic imaging},
  author={Sun, Yu and Liu, Jiaming and Xie, Mingyang and Wohlberg, Brendt and Kamilov, Ulugbek S},
  journal={IEEE Transactions on Computational Imaging},
  year={2021},
}

@inproceedings{pumarola2021d,
  title={D-nerf: Neural radiance fields for dynamic scenes},
  author={Pumarola, Albert and Corona, Enric and Pons-Moll, Gerard and Moreno-Noguer, Francesc},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{tineuvox,
  title={Fast dynamic radiance fields with time-aware neural voxels},
  author={Fang, Jiemin and Yi, Taoran and Wang, Xinggang and Xie, Lingxi and Zhang, Xiaopeng and Liu, Wenyu and Nie{\ss}ner, Matthias and Tian, Qi},
  booktitle={SIGGRAPH Asia},
  year={2022}
}

@article{maier2014comparative,
  title={Comparative validation of single-shot optical techniques for laparoscopic 3-D surface reconstruction},
  author={Maier-Hein, Lena and Groch, Anja and Bartoli, Adrien and Bodenstedt, Sebastian and Boissonnat, Guillaume and Chang, P-L and Clancy, Neil T and Elson, Daniel S and Haase, Sven and Heim, Eric and others},
  journal={TMI},
  year={2014},
}

@article{mahmoud2018live,
  title={Live tracking and dense reconstruction for handheld monocular endoscopy},
  author={Mahmoud, Nader and Collins, Toby and Hostettler, Alexandre and Soler, Luc and Doignon, Christophe and Montiel, Jose Maria Martinez},
  journal={TMI},
  year={2018},
}

@article{semmler20163d,
  title={3D reconstruction of human laryngeal dynamics based on endoscopic high-speed recordings},
  author={Semmler, Marion and Kniesburges, Stefan and Birk, Veronika and Ziethe, Anke and Patel, Rita and D{\"o}llinger, Michael},
  journal={TMI},
  year={2016},
}

@article{luegmair2015three,
  title={Three-dimensional optical reconstruction of vocal fold kinematics using high-speed video with a laser projection system},
  author={Luegmair, Georg and Mehta, Daryush D and Kobler, James B and D{\"o}llinger, Michael},
  journal={TMI},
  year={2015},
}

@article{hamlyn1,
  title={Three-dimensional tissue deformation recovery and tracking},
  author={Mountney, Peter and Stoyanov, Danail and Yang, Guang-Zhong},
  journal={IEEE Signal Processing Magazine},
  year={2010},
}

@inproceedings{hamlyn2,
  title={Soft-tissue motion tracking and structure estimation for robotic assisted MIS procedures},
  author={Stoyanov, Danail and Mylonas, George P and Deligianni, Fani and Darzi, Ara and Yang, Guang Zhong},
  booktitle={MICCAI},
  year={2005},
}

@inproceedings{hamlyn3,
  title={Real-time stereo reconstruction in robotically assisted minimally invasive surgery},
  author={Stoyanov, Danail and Scarzanella, Marco Visentini and Pratt, Philip and Yang, Guang-Zhong},
  booktitle={MICCAI},
  year={2010},
}

@inproceedings{hamlyn4,
  title={Dynamic guidance for robotic surgery using image-constrained biomechanical models},
  author={Pratt, Philip and Stoyanov, Danail and Visentini-Scarzanella, Marco and Yang, Guang-Zhong},
  booktitle={MICCAI},
  year={2010},
}

@incollection{NEURIPS2019_9015,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer},
booktitle = {NeurIPS},
year = {2019},
}

@inproceedings{fridovich2022plenoxels,
  title={Plenoxels: Radiance fields without neural networks},
  author={Fridovich-Keil, Sara and Yu, Alex and Tancik, Matthew and Chen, Qinhong and Recht, Benjamin and Kanazawa, Angjoo},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{cao2023hexplane,
  title={Hexplane: A fast representation for dynamic scenes},
  author={Cao, Ang and Johnson, Justin},
  booktitle={CVPR},
  year={2023}
}

@inproceedings{fridovich2023k,
  title={K-planes: Explicit radiance fields in space, time, and appearance},
  author={Fridovich-Keil, Sara and Meanti, Giacomo and Warburg, Frederik Rahb{\ae}k and Recht, Benjamin and Kanazawa, Angjoo},
  booktitle={CVPR},
  year={2023}
}

@article{nerfacc,
  title={Nerfacc: A general nerf acceleration toolbox},
  author={Li, Ruilong and Tancik, Matthew and Kanazawa, Angjoo},
  journal={arXiv preprint arXiv:2210.04847},
  year={2022}
}

@article{instantngp,
  title={Instant neural graphics primitives with a multiresolution hash encoding},
  author={M{\"u}ller, Thomas and Evans, Alex and Schied, Christoph and Keller, Alexander},
  journal={ToG},
  year={2022},
}

@inproceedings{tensorf,
  title={Tensorf: Tensorial radiance fields},
  author={Chen, Anpei and Xu, Zexiang and Geiger, Andreas and Yu, Jingyi and Su, Hao},
  booktitle={ECCV},
  year={2022},
}

@inproceedings{niemeyer2022regnerf,
  title={Regnerf: Regularizing neural radiance fields for view synthesis from sparse inputs},
  author={Niemeyer, Michael and Barron, Jonathan T and Mildenhall, Ben and Sajjadi, Mehdi SM and Geiger, Andreas and Radwan, Noha},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{du2021neural,
  title={Neural radiance flow for 4d view synthesis and video processing},
  author={Du, Yilun and Zhang, Yinan and Yu, Hong-Xing and Tenenbaum, Joshua B and Wu, Jiajun},
  booktitle={ICCV},
  year={2021},
}

@inproceedings{li2021neural,
  title={Neural scene flow fields for space-time view synthesis of dynamic scenes},
  author={Li, Zhengqi and Niklaus, Simon and Snavely, Noah and Wang, Oliver},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{park2021nerfies,
  title={Nerfies: Deformable neural radiance fields},
  author={Park, Keunhong and Sinha, Utkarsh and Barron, Jonathan T and Bouaziz, Sofien and Goldman, Dan B and Seitz, Steven M and Martin-Brualla, Ricardo},
  booktitle={CVPR},
  year={2021}
}

@article{ssim,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={TIP},
  year={2004},
}

@inproceedings{lpips,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}

@article{bhat2023zoedepth,
  title={Zoedepth: Zero-shot transfer by combining relative and metric depth},
  author={Bhat, Shariq Farooq and Birkl, Reiner and Wofk, Diana and Wonka, Peter and M{\"u}ller, Matthias},
  journal={arXiv preprint arXiv:2302.12288},
  year={2023}
}

@article{oneblob,
  title={Neural importance sampling},
  author={M{\"u}ller, Thomas and McWilliams, Brian and Rousselle, Fabrice and Gross, Markus and Nov{\'a}k, Jan},
  journal={ToG},
  year={2019},
}

@article{kirillov2023segment,
  title={Segment anything},
  author={Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C and Lo, Wan-Yen and others},
  journal={arXiv preprint arXiv:2304.02643},
  year={2023}
}

==> cover_letter.tex <==

Dear Editor,

We consider submitting our paper to IEEE Transactions on Medical Imaging. Our
Our paper aims at human pose imitation. Given a source character, human pose imitation aims to manipulate this avatar to present any pose with a target human’s image as a reference. 
It is incredibly challenging due to non-rigid human body motions, signiﬁcant variations in clothing textures, and self-occluded human bodies in 2D images. 
We propose Poxture, a novel human posture imitation method with neural texture, to address the aforementioned challenges. 
Our framework can fully disentangle the source character’s appearance, shape, and pose, which enjoys several advantages: 1) It can synthesize high-resolution images with detailed textures, thanks to the learned neural textures containing both visible and invisible parts and high-frequency information; 2) It can imitate complex actions with various appearances and body ﬁgures since the complete texture of the source character is acquired. 
We verify the effectiveness of our method on two challenging datasets, showing state-of-the-art results. Extensive experiments demonstrate that, given any character, our approach can manipulate this avatar imitating arbitrary posture.

All authors have read the manuscript and approved it submitted to your journal. Thank you
very much for your attention and consideration.

Yours Sincerely,
Chen Yang
AI Institute
Shanghai Jiao Tong University
Shanghai, 200240, CN



==> egbib_all.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@article{nerf,
  title={Nerf: Representing scenes as neural radiance fields for view synthesis},
  author={Mildenhall, Ben and Srinivasan, Pratul P and Tancik, Matthew and Barron, Jonathan T and Ramamoorthi, Ravi and Ng, Ren},
  journal={Communications of the ACM},
  year={2021},
}

@inproceedings{endonerf,
  title={Neural rendering for stereo 3d reconstruction of deformable tissues in robotic surgery},
  author={Wang, Yuehao and Long, Yonghao and Fan, Siu Hin and Dou, Qi},
  booktitle={MICCAI},
  year={2022},
}

@article{endo-depth-and-motion,
  title={Endo-depth-and-motion: reconstruction and tracking in endoscopic videos using depth networks and photometric constraints},
  author={Recasens, David and Lamarca, Jos{\'e} and F{\'a}cil, Jos{\'e} M and Montiel, JMM and Civera, Javier},
  journal={RA-L},
  year={2021},
}

@inproceedings{edssr,
  title={E-dssr: efficient dynamic surgical scene reconstruction with transformer-based stereoscopic depth perception},
  author={Long, Yonghao and Li, Zhaoshuo and Yee, Chi Hang and Ng, Chi Fai and Taylor, Russell H and Unberath, Mathias and Dou, Qi},
  booktitle={MICCAI},
  year={2021},
}

@article{andersson2020flip,
  title={FLIP: A Difference Evaluator for Alternating Images.},
  author={Andersson, Pontus and Nilsson, Jim and Akenine-M{\"o}ller, Tomas and Oskarsson, Magnus and {\AA}str{\"o}m, Kalle and Fairchild, Mark D},
  journal={PACMCGIT},
  year={2020}
}

@article{andersson2021visualizing,
  title={Visualizing errors in rendered high dynamic range images},
  author={Andersson, Pontus and Nilsson, Jim and Shirley, Peter and Akenine-M{\"o}ller, Tomas},
  year={2021},
  journal={Eurographics},
}

@article{stasis,
  title={StaSiS-Net: A stacked and siamese disparity estimation network for depth reconstruction in modern 3D laparoscopy},
  author={Bardozzo, Francesco and Collins, Toby and Forgione, Antonello and Hostettler, Alexandre and Tagliaferri, Roberto},
  journal={MIA},
  year={2022},
}

@article{lerplane,
  title={Neural LerPlane Representations for Fast 4D Reconstruction of Deformable Tissues},
  author={Yang, Chen and Wang, Kailing and Wang, Yuehao and Yang, Xiaokang and Shen, Wei},
  journal={MICCAI},
  year={2023}
}

@article{song2017dynamic,
  title={Dynamic reconstruction of deformable soft-tissue with stereo scope in minimal invasive surgery},
  author={Song, Jingwei and Wang, Jun and Zhao, Liang and Huang, Shoudong and Dissanayake, Gamini},
  journal={RA-L},
  year={2017},
}

@article{zhou2019real,
  title={Real-time dense reconstruction of tissue surface from stereo optical video},
  author={Zhou, Haoyin and Jagadeesan, Jayender},
  journal={TMI},
  year={2019},
}

@inproceedings{zhou2021emdq,
  title={EMDQ-SLAM: Real-time high-resolution reconstruction of soft tissue surface from stereo laparoscopy videos},
  author={Zhou, Haoyin and Jayender, Jagadeesan},
  booktitle={MICCAI},
  year={2021},
}

@article{li2020super,
  title={Super: A surgical perception framework for endoscopic tissue manipulation with surgical robotics},
  author={Li, Yang and Richter, Florian and Lu, Jingpei and Funk, Emily K and Orosco, Ryan K and Zhu, Jianke and Yip, Michael C},
  journal={RA-L},
  year={2020},
}

@inproceedings{li20213d,
  title={3D Ultrasound Spine Imaging with Application of Neural Radiance Field Method},
  author={Li, Honggen and Chen, Hongbo and Jing, Wenke and Li, Yuwei and Zheng, Rui},
  booktitle={IUS},
  year={2021},
}

@inproceedings{khan2022implicit,
  title={Implicit Neural Representations for Medical Imaging Segmentation},
  author={Khan, Muhammad Osama and Fang, Yi},
  booktitle={MICCAI},
  year={2022},
}

@inproceedings{yang2022implicitatlas,
  title={ImplicitAtlas: learning deformable shape templates in medical imaging},
  author={Yang, Jiancheng and Wickramasinghe, Udaranga and Ni, Bingbing and Fua, Pascal},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{corona2022mednerf,
  title={Mednerf: Medical neural radiance fields for reconstructing 3d-aware ct-projections from a single x-ray},
  author={Corona-Figueroa, Abril and Frawley, Jonathan and Bond-Taylor, Sam and Bethapudi, Sarath and Shum, Hubert PH and Willcocks, Chris G},
  booktitle={EMBC},
  year={2022},
}

@article{schwarz2020graf,
  title={Graf: Generative radiance fields for 3d-aware image synthesis},
  author={Schwarz, Katja and Liao, Yiyi and Niemeyer, Michael and Geiger, Andreas},
  journal={NeurIPS},
  year={2020}
}

@article{ruckert2022neat,
  title={Neat: Neural adaptive tomography},
  author={R{\"u}ckert, Darius and Wang, Yuanhao and Li, Rui and Idoughi, Ramzi and Heidrich, Wolfgang},
  journal={TOG},
  year={2022},
}

@inproceedings{fang2022curvature,
  title={Curvature-Enhanced Implicit Function Network for High-quality Tooth Model Generation from CBCT Images},
  author={Fang, Yu and Cui, Zhiming and Ma, Lei and Mei, Lanzhuju and Zhang, Bojun and Zhao, Yue and Jiang, Zhihao and Zhan, Yiqiang and Pan, Yongsheng and Zhu, Min and others},
  booktitle={MICCAI},
  year={2022},
}

@inproceedings{raju2022deep,
  title={Deep implicit statistical shape models for 3d medical image delineation},
  author={Raju, Ashwin and Miao, Shun and Jin, Dakai and Lu, Le and Huang, Junzhou and Harrison, Adam P},
  booktitle={AAAI},
  year={2022}
}

@article{sun2021coil,
  title={Coil: Coordinate-based internal learning for tomographic imaging},
  author={Sun, Yu and Liu, Jiaming and Xie, Mingyang and Wohlberg, Brendt and Kamilov, Ulugbek S},
  journal={IEEE Transactions on Computational Imaging},
  year={2021},
}

@inproceedings{pumarola2021d,
  title={D-nerf: Neural radiance fields for dynamic scenes},
  author={Pumarola, Albert and Corona, Enric and Pons-Moll, Gerard and Moreno-Noguer, Francesc},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{tineuvox,
  title={Fast dynamic radiance fields with time-aware neural voxels},
  author={Fang, Jiemin and Yi, Taoran and Wang, Xinggang and Xie, Lingxi and Zhang, Xiaopeng and Liu, Wenyu and Nie{\ss}ner, Matthias and Tian, Qi},
  booktitle={SIGGRAPH Asia},
  year={2022}
}

@article{maier2014comparative,
  title={Comparative validation of single-shot optical techniques for laparoscopic 3-D surface reconstruction},
  author={Maier-Hein, Lena and Groch, Anja and Bartoli, Adrien and Bodenstedt, Sebastian and Boissonnat, Guillaume and Chang, P-L and Clancy, Neil T and Elson, Daniel S and Haase, Sven and Heim, Eric and others},
  journal={TMI},
  year={2014},
}

@article{mahmoud2018live,
  title={Live tracking and dense reconstruction for handheld monocular endoscopy},
  author={Mahmoud, Nader and Collins, Toby and Hostettler, Alexandre and Soler, Luc and Doignon, Christophe and Montiel, Jose Maria Martinez},
  journal={TMI},
  year={2018},
}

@article{semmler20163d,
  title={3D reconstruction of human laryngeal dynamics based on endoscopic high-speed recordings},
  author={Semmler, Marion and Kniesburges, Stefan and Birk, Veronika and Ziethe, Anke and Patel, Rita and D{\"o}llinger, Michael},
  journal={TMI},
  year={2016},
}

@article{luegmair2015three,
  title={Three-dimensional optical reconstruction of vocal fold kinematics using high-speed video with a laser projection system},
  author={Luegmair, Georg and Mehta, Daryush D and Kobler, James B and D{\"o}llinger, Michael},
  journal={TMI},
  year={2015},
}

@article{hamlyn1,
  title={Three-dimensional tissue deformation recovery and tracking},
  author={Mountney, Peter and Stoyanov, Danail and Yang, Guang-Zhong},
  journal={IEEE Signal Processing Magazine},
  year={2010},
}

@inproceedings{hamlyn2,
  title={Soft-tissue motion tracking and structure estimation for robotic assisted MIS procedures},
  author={Stoyanov, Danail and Mylonas, George P and Deligianni, Fani and Darzi, Ara and Yang, Guang Zhong},
  booktitle={MICCAI},
  year={2005},
}

@inproceedings{hamlyn3,
  title={Real-time stereo reconstruction in robotically assisted minimally invasive surgery},
  author={Stoyanov, Danail and Scarzanella, Marco Visentini and Pratt, Philip and Yang, Guang-Zhong},
  booktitle={MICCAI},
  year={2010},
}

@inproceedings{hamlyn4,
  title={Dynamic guidance for robotic surgery using image-constrained biomechanical models},
  author={Pratt, Philip and Stoyanov, Danail and Visentini-Scarzanella, Marco and Yang, Guang-Zhong},
  booktitle={MICCAI},
  year={2010},
}

@incollection{NEURIPS2019_9015,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer},
booktitle = {NeurIPS},
year = {2019},
}

@inproceedings{fridovich2022plenoxels,
  title={Plenoxels: Radiance fields without neural networks},
  author={Fridovich-Keil, Sara and Yu, Alex and Tancik, Matthew and Chen, Qinhong and Recht, Benjamin and Kanazawa, Angjoo},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{cao2023hexplane,
  title={Hexplane: A fast representation for dynamic scenes},
  author={Cao, Ang and Johnson, Justin},
  booktitle={CVPR},
  year={2023}
}

@inproceedings{fridovich2023k,
  title={K-planes: Explicit radiance fields in space, time, and appearance},
  author={Fridovich-Keil, Sara and Meanti, Giacomo and Warburg, Frederik Rahb{\ae}k and Recht, Benjamin and Kanazawa, Angjoo},
  booktitle={CVPR},
  year={2023}
}

@article{nerfacc,
  title={Nerfacc: A general nerf acceleration toolbox},
  author={Li, Ruilong and Tancik, Matthew and Kanazawa, Angjoo},
  journal={arXiv preprint arXiv:2210.04847},
  year={2022}
}

@article{instantngp,
  title={Instant neural graphics primitives with a multiresolution hash encoding},
  author={M{\"u}ller, Thomas and Evans, Alex and Schied, Christoph and Keller, Alexander},
  journal={ToG},
  year={2022},
}

@inproceedings{tensorf,
  title={Tensorf: Tensorial radiance fields},
  author={Chen, Anpei and Xu, Zexiang and Geiger, Andreas and Yu, Jingyi and Su, Hao},
  booktitle={ECCV},
  year={2022},
}

@inproceedings{niemeyer2022regnerf,
  title={Regnerf: Regularizing neural radiance fields for view synthesis from sparse inputs},
  author={Niemeyer, Michael and Barron, Jonathan T and Mildenhall, Ben and Sajjadi, Mehdi SM and Geiger, Andreas and Radwan, Noha},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{du2021neural,
  title={Neural radiance flow for 4d view synthesis and video processing},
  author={Du, Yilun and Zhang, Yinan and Yu, Hong-Xing and Tenenbaum, Joshua B and Wu, Jiajun},
  booktitle={ICCV},
  year={2021},
}

@inproceedings{li2021neural,
  title={Neural scene flow fields for space-time view synthesis of dynamic scenes},
  author={Li, Zhengqi and Niklaus, Simon and Snavely, Noah and Wang, Oliver},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{park2021nerfies,
  title={Nerfies: Deformable neural radiance fields},
  author={Park, Keunhong and Sinha, Utkarsh and Barron, Jonathan T and Bouaziz, Sofien and Goldman, Dan B and Seitz, Steven M and Martin-Brualla, Ricardo},
  booktitle={CVPR},
  year={2021}
}

@article{ssim,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={TIP},
  year={2004},
}

@inproceedings{lpips,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}

@article{bhat2023zoedepth,
  title={Zoedepth: Zero-shot transfer by combining relative and metric depth},
  author={Bhat, Shariq Farooq and Birkl, Reiner and Wofk, Diana and Wonka, Peter and M{\"u}ller, Matthias},
  journal={arXiv preprint arXiv:2302.12288},
  year={2023}
}

@article{oneblob,
  title={Neural importance sampling},
  author={M{\"u}ller, Thomas and McWilliams, Brian and Rousselle, Fabrice and Gross, Markus and Nov{\'a}k, Jan},
  journal={ToG},
  year={2019},
}

@article{kirillov2023segment,
  title={Segment anything},
  author={Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C and Lo, Wan-Yen and others},
  journal={arXiv preprint arXiv:2304.02643},
  year={2023}
}
